Generalized weight properties of resultants and discriminants, and applications to projective enumerative geometry

The goal of this text is to understand and prove a formula stated by Salmon, which gives the first terms of some Taylor expansion of the discriminant of a plane algebraic curve. Salmon uses his formula to derive various enumerative quantities for surfaces in $\mathbf{P}^3$. We provide complete proofs of this formula and its enumerative applications, and extend Salmon's considerations to hypersurfaces in a projective space of arbitrary dimension. To this end, we introduce the concept of reduced discriminant, and provide a thorough study of its weight properties; the latter are deeply linked to projective enumerative geometric properties.

==> reddisc.tex <==
\chaptitle[Generalized weight properties of resultants and
discriminants]
{Generalized weight properties of resultants and discriminants,
and applications to projective enumerative geometry}
\chapauthor{Laurent Busé and Thomas Dedieu}

\startchap
\label{16.th+l-redres}

\newcommand{\no}{n\textsuperscript{o}}
\newcommand{\nos}{n\textsuperscript{os}}

% macros specifiques pour ce texte : formule Salmon
\newcommand{\taylordisc}{\smash
{(\raisebox{-.8mm}{\textpmhg{a}}\kern -.7mm)}}
% in case one want to go back to normal use:
% \newcommand{\taylordisc}{\eqref{taylor-discr}}

\def\Qc{{\mathcal{Q}}}
\newcommand{\AZ}[1][\Z]{A_{#1}}
\newcommand{\x}{\mathbf{x}}
\renewcommand{\a}{\mathbf{a}}
\newcommand{\balpha}{{\boldsymbol\alpha}}
\newcommand{\IZ}[1][\Z]{\mathfrak{I}_{#1}}
\newcommand{\wt}{\operatorname{weight}}
\newcommand{\weight}{\mathrm{weight}}
\newcommand{\conorm}[1]{\mathcal{C}_{#1}}
\newcommand{\tconorm}[1]{\tilde{\mathcal{C}}_{#1}}
\newcommand{\Tan}[1]{\mathcal{T}_{#1}}
\newcommand{\TanZ}[1]{\mathcal{T}_{#1}^{\circ}}

%\DeclareMathOperator{\Polar}{\mathrm{D}}
\newcommand{\Polar}{\mathrm{D}}
\newcommand{\dD}{\mathrm{D}}
% \newcommand{\obs-polar}[2]{\Polar_{#1}#2}
\newcommand{\obspolar}[2]{\mathrm{D} _{#1} #2}
\newcommand{\polar}[2]{\dD ^{#1} #2}
\newcommand{\TC}{\mathrm{TC}}

\newcommand{\redRes}{\operatorname{redRes}}
\newcommand{\redDisc}{\operatorname{redDisc}}

\let\oldflat\flat
\def\flat#1{\vphantom{#1}^\oldflat \kern -.1em #1}

\newcommand{\valuation}{order}

\renewcommand{\O}{\mathcal{O}}

\setdefaultenum{(i)}{}{}{}
%\setdefaultitem{---}{}{}{}

% \listedutaf

% \begin{abstract}
% 	In a book dating back to 1862, Salmon stated a formula
% giving the first terms of the Taylor expansion of the discriminant of
% a plane algebraic curve, and from it derived various enumerative quantities
% for surfaces in $\P^3$. In this text, we provide complete proofs of
% this formula and its enumerative applications, and extend Salmon's
% considerations to hypersurfaces in a projective space of arbitrary
% dimension. 
% To this end, we extend reduced elimination theory by
% introducing the concept of reduced discriminant, and provide a
% thorough study of its weight properties; the latter are deeply linked to
% projective enumerative geometric properties. Then, following Salmon's
% approach, we compute the number of members of a pencil of hyperplanes
% that are bitangent to a fixed projective hypersurface.
% Some other results in the
% same spirit are also discussed.
% \end{abstract}



\startcontents[16.redres]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[16.redres]{}{1}[2]{}

\bigskip

In his wonderful book \cite{salmon2_16}, first published in 1862, 
Salmon casually gives the leading term of some Taylor
expansion of the discriminant of a plane algebraic curve.
Consider the curve $\V(F) \subset \P^2$;
in a suitable system of homogeneous coordinates
$(X\!:\!Y\!:\!Z)$, its equation $F$ has
the form
\[
F(X,Y,Z)=TZ^{d-1}Y+\frac{1}{2}Z^{d-2}(AX^2+2BXY+CY^2)+\sum_{k \geq 3}
Z^{d-k} F_{k}(X,Y)=0,
\]
where each polynomial $F_{k}(X,Y)$ is homogeneous of degree $k$ in
$X,Y$, and $T,A,B,C$ are coefficients of $F$.
Salmon states, without any explanation or reference,
that the discriminant of $F$ is of the form
\begin{equation*}
\raisebox{.7mm}{\smash{(\raisebox{-.8mm}{\textpmhg{a}}\kern -.7mm)}}
\hskip \textwidth minus \textwidth
\Disc(F)=
T^2A(B^2-AC)^2\,\Phi+T^3\,\Psi,
\hskip \textwidth minus \textwidth
\hphantom{(\textpmhg{a})}
\end{equation*}
where $\Phi$ is ``the discriminant when $T$ vanishes''
(and $\Psi$ is some polynomial in the coefficients of $F$)
\cite[\S~605]{salmon2_16}.
This note arose as an attempt to understand and prove this formula.

We introduce the
\emph{reduced discriminant} of a hypersurface (or homogeneous
polynomial), of which $\Phi$ is an instance, it turns out.
It is deeply linked with the \emph{reduced resultant}, introduced by
Zariski in \cite{zariski_16}, in 1936 long after Salmon.
Of course, when $T$ is zero, $\V(F)$ is singular at the point $(0:0:1)$,
no matter the other coefficients of $F$, and correspondingly $\Disc(F)$
vanishes identically.
The polynomial $\Phi$, in fact, vanishes at those values of the 
coefficients of $F$ for which the curve $\V(F)$ has some additional
singularity besides the point $(0:0:1)$.
The reduced discriminant generalizes this to the case when $F$ has a
singular point of arbitrary multiplicity $s$.
Somehow built in the theory is a general form of
Formula~\taylordisc{}. We show how to get \taylordisc{} specifically
(in fact with a normalization factor $-\frac 1 2$,
which is probably irrelevant for Salmon), and generalize
the formula for
hypersurfaces of arbitrary dimension, see Section~\ref{s:app-to-Salmon}.
This is certainly what Salmon has in mind, although arguably only for
$s=2$, and possibly only empirically.
It has since then been apparently completely
forgotten; we have only found a faint trace
of these ideas in Salmon's works, see
Paragraph~\ref{p:salmon-hist}. We point out that the reduced
discriminant is a particular instance of the theory of toric
discriminants studied in \cite{GKZ-16}, which is more general in terms of
the family of hypersurfaces that can be considered. 
The methodology that we develop here in the specific setting of the
reduced 
discriminant is different from the theory of toric discriminants, and
we found it particularly well adapted, if not necessary, to tackle
Salmon's formula.

Salmon then uses Formula~\taylordisc{} to derive various
enumerative quantities for surfaces
$S \subset \P^3$.
In particular, he computes the number of bitangent planes
passing through a fixed general point $p \in \P^3$.
We explain his method, which involves a remarkable trick in
elimination theory, and generalize it for hypersurfaces of arbitrary
dimension.
Salmon's strategy is to consider a pencil of planes with center a line
tangent to the surface $S$ at some point $p'$;
this pencil contains a finite number of planes tangent to $S$,
among which the tangent plane at $p'$ counts with multiplicity $2$ in
general,
and with greater multiplicity if it has some special feature,
\eg if it is a bitangent plane.
In an appropriate setting, this multiplicity is the
\valuation{} in $T$
of the polynomial in \taylordisc{}, and the game is to understand the
conditions on the point $p'$ that make this multiplicity jump.
In the upshot we get, indirectly from the reduced discriminant $\Phi$,
a curve in $S$ parametrizing those points $p'$ such that the tangent
plane at $p'$ is a bitangent plane; following Salmon, we call it the 
\emph{node-couple curve}.
There are other well-known ways to compute the number of bitangent
planes to a surface in $\P^3$
(see, \eg \cite{13.th-classic}). 
The present method has the advantage of being core level: it is only a
study of homogeneous polynomials and their discriminants.

% Let us list a few points in favour of
% Salmon's technique. First of all it is the natural approach, and does
% not involve any trick. A concrete manifestation of this is that
% Salmon's technique gives more than a mere degree: it shows the
% existence of a node-couple hypersurface, the intersection of which
% with the surface under consideration is the locus of tangency points
% of bitangent planes (see Theorem~\ref{t:node-couple}).
% Moreover, it works over an arbitrary algebraically closed field of
% characteristic zero, and can be carried out for a hypersurface in a
% projective space of arbitrary dimension, as we observe in the present
% text. 

% Indeed, we prove the following. 
% Let $X \subset \P^n$ be a hypersurface. In a suitable system of
% homogeneous coordinates, it is defined by a homogeneous polynomial of
% the form
% \[
% f(x_0,x_1,\ldots,x_n) = 
% T x_0 ^{d-1} x_n
% + \sum _{k \geq 2} x_0^{d-k} f_k(x_1,\ldots,x_n),
% \]
% and we prove in \ref{p:taylor-discr-arbdim} that one has
% \[
% \Disc(f) = 
% T^2 \Disc (\bar f_2) \Disc(f_2)^2 \redDisc (f) \mod T^3,
% \]
% where $\bar f_2(x_1,\ldots,x_{n-1})=f_2(x_1,\ldots,x_{n-1},0)$,
% and $\redDisc(f)$ is the \emph{reduced discriminant} of $f$ with
% respect to the truncation at the order $d-2$ in the variable $x_0$,
% see Definition~\ref{def:disc}. From this we are able to show that,
% under suitable smoothness and transversality assumptions, the number
% of bitangent hyperplanes to $X$ passing through $n-2$ general points
% in $\P^n$ is
% \[
% \frac 1 2 d (d-1)^{n-2}
% (d-2) 
% \Bigl(
% d \cdot \frac {(d-1)^{n}-1} {d-2} -3(n+1)
% \Bigr)
% \]
% (see Theorem~\ref{T:bitg-arbdim}).

The present text includes two other projective enumerative
computations taken from Salmon's book;
they both fit in the framework of what we would call
\emph{reduced elimination theory}.
The first one gives the number of bitangent lines to a surface in
$\P^3$ through a general point.
We generalize it in two ways:
to the enumeration of lines in $\P^n$ having contact of the form
$2p+(n-1)q+\cdots$ with a hypersurface on the one hand,
and to the enumeration of bitangent codimension 2 linear spaces on the
other hand. While Salmon's computation and the first generalization
do not involve openly the reduced discriminant (thanks to
the existence of a cheap substitute in the two indeterminates case),
it is essential for the latter generalization.
The second computation is that of the degree of the
\emph{flecnodal curve} of a surface $S\subset \P^3$, which is the
locus of points $p$ at which the tangent plane cuts out a curve
with one of its two branches at $p$ that has an inflection point
(equivalently, there is a line having contact order with $S$ at $p$ at
least $4$).
We present here Salmon's ideas, noting that this computation is
carried out in modern standards and in arbitrary dimension in
\cite{BASW-16}.

\bigskip
We also give a synthetic account of the theory of resultants and
discriminants, in its modern form worked out by Jouanolou, see,
\eg \cite{J91}.
On the one hand this is necessary for us to develop the theory of the
reduced discriminant
(the reduced resultant had already been treated
by Ould~Mohamdi in \cite{OM88}, under the direction of Jouanolou;
note, however, that passing from the resultant to the discriminant is
not straightforward, see, \eg, the comments after
Definition~\ref{defn:reddisc}).
On the other hand, we believe this text is a good occasion to make
Jouanolou's formalism accessible to the XXI\textsuperscript{st}
century classical algebraic geometer.

We put particular focus on the homogeneity properties of the
resultants and discriminants,
with respect to various gradings.
They are indeed essential for the enumerative applications, and we
give numerous illustrations, including a proof of Bezout's theorem and
the computation of the degree of the dual of a smooth hypersurface.
Beyond that, they are central in the theory of reduced resultants and
discriminants, see Theorem~\ref{T:red-Zgrad}
and Corollary~\ref{cor:generalizedSalmonFormula}, and indeed the key
to Formula~\taylordisc{} and its generalizations.

% \medskip
% The article is organized as follows.
% In Section~\ref{S:redRes}, we review the theory of the resultant
% including its various homogeneity properties, and introduce the
% reduced resultant following Zariski.
% In Section~\ref{S:redDisc} we discuss in the same fashion the ordinary
% discriminant and its reduced version; 
% in subsection~\ref{s:app-to-Salmon} we prove Salmon's formula
% \taylordisc{} and its version in arbitrary dimension.
% Section~\ref{S:salmon's-comput} is devoted to the computation by
% elimination from the latter formula of the number of bitangent
% hyperplanes to a smooth hypersurface, with emphasis on the surface
% case. 
% {\color{gray}
% The final Section~\verb.\ref{S:further}. contains the additional computations
% of the flecnodal degree and of the number of bitangent lines to a
% surface in $\P^3$.}

% This text is a slightly modified version of a chapter of the
% forthcoming proceedings of the Seminar on Degenerations and
% enumeration of curves on surfaces held in Roma ``Tor Vergata''
% 2015--2017.
% The main modification consists in the inclusion of
% subsection~\ref{s:polarity} on polarity to make the text more
% self-contained.

\medskip
ThD thanks Ragni Piene and Israel Vainsencher for their
interest, and for suggesting he talk with LB;
he also thanks François Lê for sharing some insights on Salmon's work.
LB is grateful to Alexandru Dimca for useful discussions on
Milnor number and for indicating the reference \cite{FuTo04}.
We both thank the referees for their helpful observations.


\paragraph{Notation}
Let $\k$ be a commutative ring, $n\geq 1$ be an integer,
and $\bX:=(X_0,X_1,\ldots,X_n)$ be a sequence of indeterminates. 
Given a multi-index
$\balpha:=(\alpha_0,\alpha_1,\ldots,\alpha_n)\in \N^n$, we denote by
$\bX^\balpha$ the monomial
$X_0^{\alpha_0}X_1^{\alpha_1}\ldots X_n^{\alpha_n}$, and 
set $|\balpha|=\sum_{i=0}^n \alpha_i$.

\begin{definition}
\label{d:order}
Given a grading 
$\k[\bX] = \bigoplus_{d \geq 0} \k[\bX]_d$,
the \emph{order} of a polynomial $F\in \k[\bX]$ is the largest integer
$e$ such that 
$F \in \bigoplus_{d \geq e} \k[\bX]_d$.

We will usually consider gradings obtained by assigning a
\emph{weight} $w_i$ to each indeterminate $X_i$:
the degree $d$ homogeneous piece $\k[\bX]_d$ is then generated by all
monomials $\bX^\balpha$ such that $\sum_{i=0}^n \alpha_i w_i = d$.

Given a subset $I \subset \{1,\ldots,n\}$, the \emph{order}
of a polynomial $F$
\emph{in the indeterminates $X_i$, $i\in I$,} is the order of $F$ with
respect to the grading obtained by assigning to $X_i$ the weight $1$
if $i \in I$, and the weight $0$ if $i \not\in I$.
\end{definition}


Beware that $\k$ itself will often be a polynomial ring, and we will
consider gradings and orders both on $\k[\bX]$ and on $\k$ itself.


\section{Reduced resultant}
\label{S:redRes}


Let $F_1,\ldots,F_{n+1}$ be $n+1$ homogeneous polynomials in the
indeterminates $X_0,X_1,\ldots,X_n$. They define a collection of $n+1$
hypersurfaces in the projective space $\P^{n}$,
and the intersection of these $n+1$ hypersurfaces is
empty if $F_1,\ldots,F_{n+1}$ are general.
In fact, the emptiness of this intersection
is characterized by the non-vanishing of the resultant
$\Res(F_1,\ldots,F_{n+1})$ of these polynomials (see \S \ref{s:res}). 
Thus, the resultant characterizes those collections of homogeneous
polynomials that have a common non-trivial root.
The purpose of the \emph{reduced resultant}
is similar:
one still considers $n+1$ homogeneous polynomials
$F_1,\ldots,F_{n+1}$, but this time one assumes that they
have a common non-trivial root; then the reduced resultant will
characterize those collections of polynomials having an additional
common non-trivial root.
It has been introduced by Zariski \cite{zariski_16}; a
more complete and modern treatment is given in \cite{OM88}. 

In what follows, we use the resultant of multivariate homogeneous
polynomials as developed in \cite{J91} (see also
\cite{CLO98,demazure,GKZ-16}).
An introduction and a brief recap are given in Section~\ref{s:res}
below.



\subsection{Inertia forms and the ordinary multivariate resultant}
\label{s:res}

We follow the beautiful presentation in \cite[Chapter~XI]{vdW} (beware
that this Chapter on Elimination Theory has disappeared in later
editions).

\paragraph{Saturation of a homogeneous ideal}
We recall the following for the convenience of the reader; 
see, \eg \cite[Lecture~5]{harris_16} or
\cite[Exercise~II.5.10]{hartshorne_16} for more details.
The \emph{saturation} of a homogeneous ideal
$I \subset \k[\bX]$ is the homogeneous ideal
\begin{equation}
\label{not:saturation}
\begin{aligned}
\bar I &= \bigl\{ F \in \k[\bX]:
\forall i=0,\ldots,n,\  
\exists N_i\ \text{such that}\ X_i^{N_i} F \in I 
\bigr\}
\\
&= I : (X_0,\ldots,X_n)^\infty.
\end{aligned}
\end{equation}

For sufficiently large $m$, the graded pieces $I_m$ and $\bar I_m$ are
equal. Moreover, for two homogeneous ideals $I$ and $J$, the following
three propositions are equivalent:
\begin{noindparaenum}
\item $\bar I = \bar J$;
\item $I_m=J_m$ for sufficiently large $m$;
\item $I\cdot \k[\bX,\frac 1 {X_{i}}]=
J \cdot \k[\bX,\frac 1 {X_{i}}]$
for all $i=0,\ldots,n$.
\end{noindparaenum}
In other words, a subscheme $V \subset \P^n_\k$ is defined 
(scheme-theoretically) by a homogeneous ideal $I \subset \k[\bX]$ if and
only if the saturation $\bar I$ equals the homogeneous ideal $I_V$ of
$V$. 
For example, for all $F \in \k[\bX]$, the two ideals
$(F)$ and $(X_0F, \ldots, X_nF)$ define the same subcheme of $\P^n_\k$
(and we recommend that the reader check it for themselves).

In particular, if $\k$ is a field, a subscheme $V \subset \P^n_\k$
defined by a homogeneous ideal $I$ is empty if and only if the degree
$0$ piece $\bar I_0$ is non-zero: this is the homogeneous
Nullstellensatz! (see also \cite{CT78}). On the other hand, the
non-emptiness of $V$ is equivalent to the existence of a point in
$V(\k')$ for some finite field extension $\k'$ of $\k$.

When $\k$ is an arbitrary commutative integral domain,\footnote
{this arguably unconventional notation is used ubiquitously by
  Jouanolou.}
the vanishing of $\bar
I_0$ is equivalent to the scheme-theoretic image of the map 
$V \to \Spec(\k)$ being equal to the whole $\Spec(\k)$. Indeed, the
subscheme of $\Spec(\k)$ defined by 
$\bar I_0$ coincides as a set with the image of $V \to \Spec(\k)$
---~this is the proof that projective morphisms are closed~---, 
and moreover $\bar I_0$ defines the scheme-theoretic image of $V \to
\Spec(\k)$ (see, \eg \cite[\S 1]{J91} for more details).

\paragraph{}
\label{par:resnotation}
Let $d_1,\ldots,d_r$ be positive integers.
For all $j=1,\ldots,r$, we consider the \emph{generic}
homogeneous degree
$d_j$ polynomial in the indeterminates $\bX = (X_0,\ldots,X_n)$
\[
F_j:=\sum_{|\balpha|=d_j}U_{j,\balpha}\bX^\balpha.
\]
``Generic'' refers to the fact that the coefficients of the $F_j$'s
are indeterminates;
indeed, $F_j$ is an incarnation of the generic point, in the sense
of schemes, of the affine space parametrizing homogeneous degree $d_j$
polynomials.

We let $\AZ$ be the algebra generated by the indeterminates
coefficients of the $F_j$'s, i.e.,
we set $\AZ:=\Z\bigl[ U_{j,\balpha} \bigr]
_{j=1,\ldots,r, \, |\balpha|=d_j}$.
Thus, $F_j \in \AZ{}[\bX]$ for all 
$j=1,\ldots,r$.

Let $\k$ be a commutative ring,
and let $u_{j,\balpha} \in \k$ for
all $j=1,\ldots,r$ and $|\balpha| = d_j$.
For all $T\in \AZ{}[\bX]$,
we denote by $T(u_{j,\balpha}) \in \k[\bX]$ the polynomial obtained
by evaluating the indeterminates $U_{j,\balpha}$ at $u_{j,\balpha} \in
\k$ for all $j=1,\ldots,r$ and $|\balpha| = d_j$
in the polynomial $T$.



\begin{definition}
An \emph{inertia form} for the polynomials $F_1,\ldots,F_r$ is an
element $T \in \AZ{}[\bX]$ such for all $i=0,\ldots,n$, there exists $N_i \in
\N$ such that $X_i^{N_i} T \in (F_1,\ldots,F_r)$.
\end{definition}


In other words, the inertia forms for $F_1,\ldots,F_r$ are the
elements of the saturation of the ideal 
$(F_1,\ldots,F_r)$ in $\AZ{}[\bX]$.
% In particular, the set of all inertia forms is a homogeneous ideal of
% $\AZ{}[\bX]$. 
We denote by $\IZ$ the ideal of all degree $0$ inertia forms for
$F_1,\ldots,F_r$; thus, in the notation introduced in
\eqref{not:saturation},
\[
  \IZ
  = \bigl( I : (X_0,\ldots,X_n)^\infty \bigr)
  \cap \AZ.
\]
Note that this is a homogeneous ideal with respect to the standard
grading on $\AZ$.
In view of the above considerations, we have the following.

\begin{theorem}
\label{T:princ-elim}
Suppose that $\k$ is a field, and
let $u_{j,\balpha} \in \k$ for
for all $j=1,\ldots,r$ and $|\balpha| = d_j$.
Consider the polynomials 
$F_1(u_{1,\balpha}),\ldots,F_r(u_{r,\balpha}) \in \k[\bX]$.
The two following propositions are equivalent:
\begin{noindparaenum}
\item\label{c:non-empty}
the ideal $\bigl(F_1(u_{1,\balpha}),\ldots,
F_r(u_{r,\balpha})\bigr)$ defines a non-empty subscheme of $\P^n_\k$;
\item\label{c:vanish-inert}
for all $T \in \IZ$,
$T(u_{j,\balpha})=0$.
\end{noindparaenum}
\end{theorem}

This tells us that a given specialization to a field of the
polynomials $F_j$ 
defines a non-empty subscheme if and only if all the constants in the
saturation of $(F_1,\ldots,F_r)$ vanish in this
specialization (see also \cite{CT78}).
Note that for all $T \in \IZ$, one has
$T(u_{j,\balpha}) \in \k$,
since $T$ has degree $0$ in $\bX$.

\begin{example}
Set $n=1$, and let $F_1 = U_{1,0} X_0 + U_{1,1} X_1$
and $F_2 = U_{2,0} X_0 + U_{2,1} X_1$.
Then $R = U_{1,0} U_{2,1}-U_{1,1}U_{2,0}$ is a degree $0$ inertia form
of $F_1$ and $F_2$, as indeed
\[
  X_0 R = U_{2,1} F_1 - U_{1,1}F_2
  \et
  X_1 R = U_{1,0} F_2 - U_{2,0}F_1.
\]
We thus recover the usual determinant of two linear forms.
We recommend that the reader come back to this example when we
introduce various gradings on $\AZ$ later on.
\end{example}

We emphasize that in general the
subscheme of $\Spec(\k)$ defined by the specialization of $\IZ$
coincides only set-theoretically with the scheme-theoretic
image of $V \to \Spec(\k)$
(see \cite[\S 3, Remarque~1]{demazure} and \cite[\S 1]{J91}),
which is the reason why we assume that $\k$ is a field in
Theorem~\ref{T:princ-elim}.
If $\k$ is an arbitrary commutative ring, what is indeed true is that
the subscheme defined by the $F_j(u_{j,\alpha})$'s
surjects onto $\Spec(\k)$ as a set
if and only if
${\IZ \otimes _{\AZ} \k}$ is contained in the nilradical 
$\sqrt {(0)}$ of $\k$, but this says nothing more than 
Theorem~\ref{T:princ-elim}. 


\begin{theorem}[see {\cite[\S 2.1]{BJ14}}]
The ideal of inertia forms for $F_1,\ldots,F_r$ is prime, and so is the ideal $\IZ \subset \AZ$ of inertia forms of degree 0.
\end{theorem}

\noindent
The \emph{resultant situation} is when we consider $n+1$ homogeneous
equations in $\P^n$.

\begin{theorem}
\label{T:res}
If $r=n+1$, the ideal $\IZ$ is principal. 
Up to sign it has a unique generator,
which is an irreducible element of $\AZ$;
we denote it by $\Res_{d_1,\ldots,d_{n+1}} \in \AZ$.

Moreover, 
for all $k \in \intint 1 {n+1}$, $\Res_{d_1,\ldots,d_{n+1}}$ is
homogeneous of degree
$\prod _{j \neq k} d_j$ with respect to the coefficients of the
polynomial $F_k$, i.e., with respect to the indeterminates $U_{k,\balpha}$,
$|\balpha| = d_{k}$ (all assumed to have weight one).
\end{theorem}


Let $f_1,\ldots, f_{n+1} \in \k[\bX]$ be polynomials of
respective degrees $d_1,\ldots,d_{n+1}$. They are specializations
$F_1(u_{1,\balpha}),\ldots, F_r(u_{r,\balpha})$
of
$F_1,\ldots,F_{n+1} \in \AZ{}[\bX]$ respectively,
for an appropriate canonical choice of 
$u_{j,\balpha} \in \k$, for all $j=1,\ldots,n+1$ and
$|\balpha| = d_{k}$. We let $\Res(f_1,\ldots, f_{n+1})
\in \k$ 
(or $\Res_{d_1,\ldots,d_{n+1}}(f_1,\ldots, f_{n+1})
\in \k$, if
we want to emphasize the dependency on the degrees) be the
corresponding specialization of $\Res_{d_1,\ldots,d_{n+1}} \in \AZ$. The multi-homogeneity property stated in the above theorem may then be
rephrased as follows: for all $\lambda \in \k$, 
\[
\Res_{d_1,\ldots,d_{n+1}} (f_1,\ldots, 
\lambda f_{k}, \ldots, f_{n+1})
= \lambda^{d_1\cdots d_{k-1} d_{k+1} \cdots d_{n+1}}\,
\Res_{d_1,\ldots,d_{n+1}} (f_1,\ldots, 
f_{k}, \ldots, f_{n+1}).
\]
The sign indeterminacy in the definition of
$\Res_{d_1,\ldots,d_{n+1}}$ is usually removed by imposing the
normalizing equality $\Res(X_0^{d_0},\ldots,X_n^{d_n})=1$. 


\paragraph{Divisibility property
{\normalfont (see, \eg \cite[\S 5.6]{J91})}}
\label{res:divisibility}
Let $F_1,\ldots, F_{n+1}$ and $ G_1,\ldots, G_{n+1}$ be two sequences of homogeneous polynomials in $\k[\bX]$  such that we have the inclusion of ideals of $\k[\bX]$,
$$ (G_1,\ldots, G_{n+1}) \subset (F_1,\ldots, F_{n+1}).$$
Then,
$\Res(F_1,\ldots, F_{n+1})$ divides 
$\Res(G_1,\ldots, G_{n+1})$ in $\k$.


\bigskip
Besides its ordinary multi-homogeneity property
given in Theorem~\ref{T:res}, the
resultant has other homogeneous structures that we call ``weight
properties'' to emphasize that the grading of the coefficient ring
$\AZ$ is not the standard one.

\begin{proposition}[see {\cite[\S 5.13.2]{J91}}]
\label{res:quasihom.a}
In the notation of Paragraph~\ref{par:resnotation},
let $k$ be an integer in 
$\intint 0 {n}$,
and consider the grading on
$\AZ=
\Z[U_{j,\balpha}] _{j=1,\ldots,n+1,\, |\balpha|=d_j}$
% \Z[U_{j,\balpha} : j=1,\ldots,r, \, |\balpha|=d_j]$
defined by 
\begin{equation}\label{eq:gradingres1}
	\weight(U_{j,\balpha})=\alpha_{k}.
\end{equation}
In this grading, the resultant
$\Res_{d_1,\ldots,d_{n+1}}$ is homogeneous of degree
$d_1d_2\cdots d_{n+1}$.
\end{proposition}


\paragraph{}
\label{p:bezout}
Bezout Theorem, which counts the number of roots of a finite
complete intersection scheme in a projective space, and thus is the
mother of all statements in projective enumerative geometry, can be
deduced from this property. This goes as follows.

Consider $n$ homogeneous polynomials
$F_1,\ldots,F_n \in \k[X_0,\ldots,X_n]$, of degrees $d_1,\ldots,d_n$
respectively. The idea is to project $\P^n$ to $\P^1$ from a
codimension $2$ linear space, in order to reduce to
plain polynomials in one
indeterminate only, \ie homogeneous polynomials in two
indeterminates. We thus consider
\begin{equation}
\label{projBezout}
  \tilde F_j\, (T_0,T_1,\ldots,T_{n-1})
  = F_j\, \bigl(T_0X_0,\, T_0X_1,\, T_1, \ldots, T_{n-1} \bigr)
  \in \k[X_0,X_1][T_0,\ldots,T_{n-1}]
\end{equation}
for all $j=1,\ldots,n$.
A point $(x_0:x_1) \in \P^1_\k$ sits in the projection of
$\V(F_1,\ldots,F_n) \subset \P^n$ if and only if the
specializations of $\tilde F_1,\ldots, \tilde F_n$, obtained
by specializing $X_0$ and $X_1$ to $x_0$ and $x_1$
respectively,
have a common zero in $\P^{n-1}$.
We thus consider the resultant
of $\tilde F_1,\ldots, \tilde F_n$
with respect to the indeterminates $T_0,\ldots,T_{n-1}$,
\[
  \Res \bigl( \tilde F_1,\ldots, \tilde F_n \bigr)
  \in \k[X_0,X_1].
\]
Writing
$F_j = \sum_{|\balpha|=d_j} u_{j,\balpha} \bX^\balpha$,
one has
\[
  \tilde F_j = \sum_{|\balpha|=d_j}
  \bigl(u_{j,\balpha} X_0^{\alpha_0} X_1^{\alpha_1} \bigr)\,
  T_0 ^{\alpha_0+\alpha_1} T_1^{\alpha_2} \cdots T_{n-1}^{\alpha_n}.
\]
Thus,
$\tilde F_j$ has degree $d_j$ in $T_0,\ldots,T_{n-1}$, and its
coefficient in the monomial
$T_0 ^{\tilde \alpha_0} T_1 ^{\tilde \alpha_1} \cdots
T_{n-1} ^{\tilde \alpha_{n-1}}$ is a degree $\tilde \alpha_0$
homogeneous polynomial in
$X_0,X_1$.

Then, it follows from the above Proposition~\ref{res:quasihom.a} that
\[
  \Res_{d_1,\ldots,d_n} \bigl( \tilde F_1,\ldots, \tilde F_n \bigr)
  \in \k[X_0,X_1]
\]
is homogeneous of degree $d_1\cdots d_n$.
Therefore,
$\V\bigl(\Res ( \tilde F_1,\ldots, \tilde F_n )\bigr)
\subset \P^1_\k$ consists of  $d_1\cdots d_n$ points, counted with
multiplicities. 
One may then conclude that $\V(F_1,\ldots,F_n) \subset \P^n_\k$
itself consists of $d_1\cdots d_n$ points,
by the classical arguments used to prove
Bezout's theorem for the intersection of two plane curves,
see \eg
\cite[\S 4.5]{italEMS-16}.

\bigskip
The following is a parent of the weight property given in
Proposition~\ref{res:quasihom.a} above.
It is proven in \cite[\S 5.13]{J91} as well.

\begin{proposition}
\label{res:quasihom.b}
In the same situation as in Proposition~\ref{res:quasihom.a} above,
consider the grading on $\AZ$ defined by
\begin{equation}\label{eq:gradingres2}
\weight(U_{j,\balpha})=d_j-\alpha_{k}.
\end{equation}
In this grading, the resultant $\Res_{d_1,\ldots,d_{n+1}} \in \AZ$ is
homogeneous of degree 
$nd_1d_2\cdots d_{n+1}$.
\end{proposition}


One may also use the following corollary, based on the standard homogeneity of the resultant in Theorem~\ref{T:res}, to obtain additional weight properties from \ref{res:quasihom.a} and \ref{res:quasihom.b}.

\begin{corollary}
\label{p:further-wt}
Assume that the resultant
$\Res_{d_1,\ldots,d_{n+1}}$
is homogeneous of degree
$\delta$ for the grading on $\AZ$ defined by
$\weight(U_{j,\balpha}) = w_{j,\balpha}$.
Let $r_1,\ldots,r_{n+1} \in \Z$.
For the new grading on $\AZ$
defined by $\weight(U_{j,\balpha}) = w_{j,\balpha}+r_j$,
the resultant $\Res_{d_1,\ldots,d_{n+1}}$
is homogeneous of degree
\[
\delta + \sum _{1 \leq k \leq n+1} 
\Bigl(
r_k \, \prod\nolimits _{j\neq k} d_j
\Bigr).
\]
\end{corollary}

\begin{proof}
Let $k \in \intint 1 {n+1}$.
Since the resultant is homogeneous of degree 
$\prod _{j\neq k} d_j$ with respect to the indeterminates
$( U_{k,\balpha} )_{|\balpha| = d_k}$
(for the standard grading), a shift by $r_k$ in the weights of all the
indeterminates
$( U_{k,\balpha} )_{|\balpha| = d_k}$
induces a shift by 
$r_k \, \prod _{j\neq k} d_j$ in the degree of the resultant.
\end{proof}



\subsection{The reduced resultant}\label{subsec:redres}

We shall now explain how to adapt the ideas of the previous paragraph
to develop the theory of the reduced resultant. 
We refer to \cite{zariski_16} and \cite{OM88} for the details and proofs.
Somehow, this is a generalization of the following toy example.

\begin{example}[projection of a complete intersection from one of its
points]
\label{ex:toy}
Let $F,G \in \k[\bX]$ be two homogeneous polynomials of degrees $a$ and
$b$, defining a complete intersection $V \subset \P^n$,
and suppose one wants to
project $V$ from a point $p_0 \in \P^n$. 
Assume for simplicity that $\k$ is an algebraically closed field.  
We may take
$p_0=(1:0:\ldots:0)$. Then, we consider the two polynomials
\begin{equation}
\label{projectCI}
\begin{aligned}
F(T,X_1,\ldots,X_{n})&=F_0 T^a + F_1 T^{a-1} + \cdots + F_a \\
\text{and} \quad
G(T,X_1,\ldots,X_{n})&=G_0 T^b + G_1 T^{b-1} + \cdots + G_b  
\end{aligned}
\end{equation}
in $\k[X_1,\ldots,X_{n}][T]$.
We are abusing notation here, as one should consider instead the two
polynomials $F(T,S\,X_1,\ldots,S\,X_{n})$ and 
$G(T,S\,X_1,\ldots,S\,X_{n})$ that are homogeneous in the couple of
indeterminates $(S,T)$.
Moreover, beware that \eqref{projectCI} above is written ``in reverse 
order'' with respect to what we did when discussing Bezout
Theorem, see \eqref{projBezout}.

If $p_0 \not\in V$, the point $(x_1:\ldots:x_{n}) \in \P_\k^{n-1}$
belongs to the projection of $V$ from $p_0$ if and only if the two
polynomials in  
\eqref{projectCI} have a common root in $\P^1$, hence the equation of the
projection is given by 
\[
\Res_{a,b}(F,G) \in \k[X_1,\ldots,X_{n}],
\]
which is homogeneous of degree $ab$ in the indeterminates
$(X_1,\ldots,X_{n})$ by Proposition~\ref{res:quasihom.b}, as the
polynomials 
$F_i$ are homogeneous of degree $i$ in  $\k[X_1,\ldots,X_{n}]$. 

On the other hand, if $p_0 \in V$ then, letting $a'$ and $b'$ be the
respective multiplicities of $p_0$ in the hypersurfaces $\V(F)$ and
$\V(G)$, one has
\[
F_0 = \cdots = F_{a'-1} 
= G_0 = \cdots = G_{b'-1}
=0,
\]
so that \eqref{projectCI} becomes
\begin{equation}
\label{projectCI-red}
\begin{aligned}
F(T,X_1,\ldots,X_{n})&=F_{a'} T^{a-a'} + \cdots + F_a = \flat F \\
\text{and} \quad
G(T,X_1,\ldots,X_{n})&=G_{b'} T^{b-b'} + \cdots + G_b = \flat G.
\end{aligned}
\end{equation}
It follows that the equation of the projection of $V$ from $p_0$ is
given by 
\[
\Res_{a-a',b-b'}(\flat F,\flat G) \in \k[X_1,\ldots,X_{n}].
\]
We shall see later on that this polynomial is the
\emph{reduced resultant} of $F$ and $G$ 
truncated at orders $a-a'$ and $b-b'$ respectively, as polynomials in the
indeterminate $T$. It is a homogeneous polynomial of degree $ab-a'b'$ in
$(X_1,\ldots,X_{n})$:
indeed, the coefficient of 
$\flat F$ (respectively, $\flat G$) in $T^i$
is a homogeneous polynomial in 
$(X_1,\ldots,X_n)$ of degree
$a-i=\deg_T (\flat F)-i+a'$
(respectively, $b-i=\deg_T (\flat G)-i+b'$).
Therefore, Corollary~\ref{p:further-wt} applied to
the grading of Proposition~\ref{res:quasihom.b} gives that
$\Res_{a-a',b-b'}(\flat F,\flat G)$ is homogeneous of degree
\[
(a-a')(b-b') + a'(b-b') + b'(a-a')
= ab - a'b',
\]
as we had announced. 
This weight property is an instance of
that given in Corollary~\ref{par:weightredres},
which applies to reduced resultants in general.
\end{example}


\paragraph{}
\label{par:redresnotation}
Let 
$d_1,\ldots,d_{n+1}$ be positive integers.
For all $j \in \intint{1}{n+1}$, we consider the generic homogeneous
degree $d_j$ polynomial $F_j$, which we write as
\[
F_j=\sum_{|\balpha|=d_j}U_{j,\balpha}\bX^\balpha=\sum_{k=0}^{d_j}
X_0^{d_j-k}\,F_{j,k}(X_1,\ldots,X_{n}).
\]
Thus, for all $k=0,\ldots,d_j$, the polynomial
$F_{j,k}$ is a degree $k$ homogeneous element of
$\AZ{}[X_1,\ldots,X_n]$. 
We fix integers $s_j \in \intint 1 {d_j}$ for all $j=1,\ldots,n+1$.
The \emph{truncation} of $F_j$ at order $d_j-s_j$ with respect to $X_0$ 
is the polynomial
\[
H_j=\sum_{k=s_j}^{d_j} X_0^{d_j-k}
F_{j,k}=X_0^{d_j-s_j}F_{j,s_j}+\cdots+X_0F_{j,d_j-1}+F_{j,d_j} \in \AZ{}[\x].
\]
This definition gives a special role to the indeterminate $X_0$, and
to the point $(1:0:...:0) \in \P^n$. One may thus think of the latter
as the (chosen) origin in the affine space $\P^n -\V(X_0)$, and of
$\V(X_0)$ as the hyperplane at infinity. We may occasionally use this
terminology. 


\bigskip
The purpose of reduced elimination theory is to study inertia
forms of the truncations $H_1,\ldots,H_{n+1}$ defined above.
Note that, for all $j=1,\ldots,n+1$, the truncation
$H_j$ is the generic homogeneous
polynomial of degree $d_j$ with a multiplicity $s_j$ zero in the
origin $(1:0:...:0)$.
The wish for the reduced resultant is that it is a polynomial in the
coefficients of $H_1,\ldots,H_{n+1}$, which vanishes if and only if
$H_1,\ldots,H_{n+1}$ have a non-trivial common root in addition to
that of multiplicity $s_1\cdots s_{n+1}$ at the origin.


This can be done with essentially the same strategy as in the
classical case, which we have reviewed in Section \ref{s:res}.
We will only consider the ``resultant situation'', when the number of
polynomials is $n+1$.


\begin{theorem}[{\cite[Theorem 6 and \S 8]{zariski_16} and 
\cite[Theorem II.0.5 and \S IV.0]{OM88}}]
\label{thm:redres}
	 Assume that $d_j>s_j$ for some $j \in \intint{1}{n+1}$.
The ideal of reduced inertia forms of degree 0
\[
\Qc_\Z=\bigl( (H_1,\ldots,H_{n +1}): (X_1,\ldots,X_{n})^\infty
\bigr) \cap A_\Z
\]
is a prime and principal ideal of $\AZ{}$.
The \emph{reduced resultant}, denoted
\[
\redRes_{d_1,\ldots,d_{n+1}}^{s_1,\ldots,s_{n+1}}
\in \AZ,
\]
is defined, up to sign, 
as the generator of $\Qc_\Z$; it is therefore an irreducible
element of $\AZ{}$.

Moreover, if $d_j>s_j$ for at least two distinct integers $j,j' \in
\intint{1}{n+1}$, then for all $i\in \intint{1}{n+1}$ the reduced
resultant is a homogeneous polynomial of degree
$$\frac{d_1d_2\cdots d_{n+1}}{d_i} - \frac{s_1s_2\cdots s_{n+1}}{s_i}$$
with respect to the coefficients of the polynomial $H_i$, i.e., with
respect to the indeterminates $U_{i,\balpha}$ such that $|\balpha|=d_i$
and $\alpha_0\leq d_i-s_i$.

If there is only one integer $j \in \intint{1}{n+1}$ such that
$d_j>s_j$, then the reduced resultant is equal to the resultant of the
polynomials $H_1,\ldots,H_{j-1},\, H_{j+1},\ldots,H_{n+1}$,
as polynomials in $X_1,\ldots,X_n$
only.\footnote
{if $s_j=d_j$, then $H_j = F_{j,d_j}$ is a polynomial in
  $X_1,\ldots,X_n$ only; geometrically, the polynomial
  $H_j$ defines a cone in $\P^n$ over the hypersurface defined by
$F_{j,d_j}$ in $\P^{n-1}$.}
\end{theorem}

The sign indeterminacy in the definition
of the reduced resultant can be removed by means of
Theorem~\ref{T:red-Zgrad} below,
once the sign of the ordinary resultant has been 
chosen.

Note that, in the above statement, the ideal $(H_1,\ldots,H_{n+1})$ is
saturated with respect to $(X_1,\ldots,X_n)$,
which is the defining ideal of the point $(1:0:\ldots:0)$,
whereas for the plain resultant we considered instead
the saturation with respect to the irrelevant ideal
$(X_0,X_1,\ldots,X_n)$.
Beware moreover that the polynomials
$H_1,\ldots,H_{n+1}$ are not homogeneous in the set of indeterminates
$(X_1,\ldots,X_n)$. 

The reduced resultant depends, of course, only on the
coefficients of the generic truncated polynomials
$H_1,\ldots,H_{n+1}$, and not on all 
the coefficients of the polynomials $F_1,\ldots,F_{n+1}$.
We will often
denote it by $\redRes(H_1,\ldots,H_{n+1})$ without printing the
integers $d_i$ and $s_i$, that are implicitly given by the polynomials
$H_1,\ldots,H_{n+1}$.
We may also use the notation $\redRes(F_1,\ldots,F_{n+1})$, to avoid
giving particular names to the truncation.

The reduced resultant of a
collection of polynomials $h_1,\ldots, h_{n+1} \in
\k[\bX]$
with zeros of respective multiplicities at least $s_1,\ldots,s_{n+1}$ at the
origin
is defined as the corresponding specialization of the generic
reduced resultant; it is an element in $\k$, denoted by
$\redRes(h_1,\ldots, h_{n+1})$, or possibly
$\redRes(f_1,\ldots, f_{n+1})$ depending on the context.



\paragraph{Vanishing of the reduced resultant} 
\label{p:geominterp-redres}
The reduced resultant $\redRes(H_1,\ldots,H_{n+1})$ is a polynomial in
the coefficients of the polynomials $H_j$, $j=1,\ldots,n+1$,
i.e., an element of the ring
\[
  \Z \bigl[ U_{i,\balpha} \bigr]
  _{i=1,\ldots,n+1,\,
    |\balpha|=d_i,\,
    \alpha_0\leq d_i-s_i}
  \subset \AZ{}.
\]
Its vanishing on an algebraically closed field $\k$
characterizes those collections of hypersurfaces of $\P^n_\k$ 
defined by $h_1,\ldots, h_{n+1}$
that have a further intersection point, infinitely near or not,
besides the origin $p_0 = (1\!:\!0\!:\!\ldots\!:\!0)$,
\ie those collections such that one of
the two following conditions holds:
\begin{mycpctenum}[(a)]
%	\setlength\itemsep{0em}
\item the hypersurfaces defined by
  $h_1,\ldots, h_{n+1}$
  intersect at a point which is different from $p_0$;
\item[(b)] the polynomials $f_{j,s_j}$, $j=1,\ldots,n+1$, have a
  common root in $\P^{n-1}_\k$, which means that the tangent cones
  of the hypersurfaces $\V(h_1),\ldots,\V(h_{n+1})$
  at $p_0$ have a line in common;
  equivalently, the proper transforms of $\V(h_1),\ldots,\V(h_{n+1})$
  in the blow-up 
  of $\P^n_\k$ at $p_0$ have a point in common which lies on
  the exceptional divisor.
\end{mycpctenum}
This property of the reduced resultant is proved in
\cite[Theorem 3.1, 3.2 and 3.3]{zariski_16},
and in \cite[Proposition I.1]{OM88}.


\subsection{Generalized weight properties}

In \cite{zariski_16} Zariski showed that the reduced resultant can be computed from the corresponding resultant. To obtain this property, he introduced  a generalization of the grading \eqref{eq:gradingres1} and, although the resultant is not homogeneous with respect to this new grading, he proved that its graded piece of smallest degree is connected to the reduced resultant.

\noindent
We maintain the notation of Section \ref{subsec:redres}.

\paragraph{The Zariski grading}
\label{p:Zdeg}
We define a grading on $\AZ=\Z[U_{j,\balpha}]$ by assigning for all $j$
\[
\weight(U_{j,\balpha}) = 
\begin{cases}
0 & \text{if}\ \alpha_0 < d_j-s_j \\
\alpha_0-d_j+s_j & \text{otherwise},
\end{cases}
\]
and weight $0$ to the constants.
We find it helpful to visualize this definition as follows:
\begin{equation}
\label{eq:Zariski-weight}
F_j=
 \underbrace{X_0^{d_j} F_{j,0}}
_{\text{coeffs have } \weight\ s_j}
+\, \cdots\, + \quad
\underbrace{X_0^{d_j-s_j+1}F_{j,s_j-1}}
_{\text{coeffs have } \weight\ 1}
\quad+\quad
\underbrace{X_0^{d_j-s_j}F_{j,s_j}
+\cdots+
F_{j,d_j}}
_{\text{coeffs have } \weight\ 0}
.
\end{equation}
Note in particular that the indeterminates $U_{j,\balpha}$ whose weight
equals $0$ in this grading are exactly the coefficients of the
truncation $H_j$ of the polynomial $F_j$.
The grading \eqref{eq:gradingres1} introduced in
Proposition~\ref{res:quasihom.a} is
a particular case of a Zariski grading (corresponding to $s_j=d_j$ for
all $j$), which explains the terminology ``generalized weight
properties''.


\bigskip
The main property of the Zariski grading is that it allows the
computation of the reduced resultant of $H_1,\ldots,H_{n+1}$ 
(the truncations of $F_1,\ldots,F_{n+1}$ at the orders
$d_1-s_1,\ldots,d_{n+1}-s_{n+1}$, respectively) 
from the resultant of $F_1,\ldots,F_{n+1}$. 
We need one more piece of notation to see how this goes.


\paragraph{}
\label{p:G_j}
For all $j=1,\ldots,n+1$, we let
$G_j$ be the quotient of the Euclidean division of $F_j$ by
$X_0^{d_j-s_j}$ in $\AZ{}[X_1,\ldots,X_{n}][X_0]$,
\ie
{\setlength{\multlinegap}{15mm}
\begin{multline*}
G_j \, =\,  \frac 1 {X_0^{d_j-s_j}} 
\sum _{k\leq s_j} X_0^{d_j-k}\, F_{j,k}
\, =\,  \sum _{k=0} ^{s_j} X_0^{s_j-k}\, F_{j,k}
\\
= X_0 ^{s_j}\, F_{j,0} + \cdots + X_0\, F_{j,s_j-1} + F_{j,s_j}.
\end{multline*}
}%
The polynomial $G_j$ is a generic degree $s_j$ homogeneous polynomial
in the set of variables $\bX$. Beware that $F_j$ does not equal
$H_j+X_0^{d_j-s_j}G_j$, as $F_{j,s_j}$ appears in both $H_j$ and
$G_j$:
\begin{equation}
\label{eq:F_jH_jG_j}
F_j=
\rlap{\raisebox{-1mm}{\ensuremath{
    \underbrace
    {\phantom{
        X_0^{d_j}\, F_{j,0}
        + \cdots +
        \underbrace{X_0^{d_j-s_j}\, F_{j,s_j}}
        _{\displaystyle = H_j}
      }
    }
    _{\displaystyle = X_0^{d_j-s_j}\, G_j}
  }}}
X_0^{d_j}\, F_{j,0}
+ \cdots +
\underbrace{X_0^{d_j-s_j}\, F_{j,s_j}
+\cdots+
F_{j,d_j}}_{\displaystyle = H_j}
.
\end{equation}
Also, we advise the reader to compare Displays
\eqref{eq:Zariski-weight}
and \eqref{eq:F_jH_jG_j}.


\begin{theorem}[Zariski Formula,
  {\cite[Theorem 5.1 and Theorem 5.2]{zariski_16} and
\cite[Lemme IV.1.6]{OM88}}]
\label{T:red-Zgrad}
The nonzero homogeneous piece of lowest degree with respect to the Zariski
grading of
$\Res(F_1,\ldots,F_{n+1})$ has degree $s_1s_2\cdots s_{n+1}$. 
Denote it by
$\bigl[ \Res(F_1,\ldots,F_{n+1}) \bigr] _{s_1s_2\cdots s_{n+1}}$.
\\(a) If $s_j<d_j$ for at least two distinct integers $j=j_1,j_2 \in
\intint{1}{n+1}$, then
\[
  \bigl[ \Res(F_1,\ldots,F_{n+1}) \bigr] _{s_1s_2\cdots s_{n+1}}
  =
  \Res(G_1,\ldots,G_{n+1})\cdot \redRes(H_1,\ldots,H_{n+1}).
\]
\\(b)
If there exists $j_0 \in \intint 1 {n+1}$ such that
$s_{j_0} < d_{j_0}$ and $s_j=d_j$ for all $j \neq j_0$,
then
\[
  \bigl[ \Res(F_1,\ldots,F_{n+1}) \bigr] _{s_1s_2\cdots s_{n+1}}
  = \Res(G_1,\ldots,G_{n+1})\cdot
  \redRes(H_1,\ldots,H_{n+1})^{d_{j_0}-s_{j_0}}.
\]
\end{theorem}

Note that despite appearances, there is a Zariski Formula in all
cases, because if none of the two conditions in (a) and (b) of the
above statement is verified,
then the reduced resultant is actually an ordinary resultant.

Observe that, in the Zariski grading:
(i) the coefficients of $H_1,\ldots,H_{n+1}$ all have
weight $0$,
hence $\redRes(H_1,\ldots,H_{n+1})$ is homogeneous of degree $0$;
(ii) for all $j=1,\ldots,n+1$, the coefficient of $G_j$
in $\bX^\balpha$ has weight $\alpha_0$
hence, by Proposition~\ref{res:quasihom.a},
$\Res(G_1,\ldots,G_{n+1})$ is homogeneous of weight
$s_1s_2\cdots s_{n+1}$.
Thus, indeed,
\[
  \Res(G_1,\ldots,G_{n+1})\cdot
  \redRes(H_1,\ldots,H_{n+1})^e
\]
is homogeneous of weight $s_1s_2\cdots s_{n+1}$ for all $e$.


\begin{corollary}
\label{par:weightredres}
Consider the grading of $\AZ$ defined by
\begin{equation*}
\weight(U_{j,\balpha})=d_j-\alpha_{0}.
\end{equation*}
With respect to this grading,
$\redRes(H_1,\ldots,H_{n+1})$ 
is homogeneous of degree
\[
  n(d_1\cdots d_{n+1}-s_1\cdots s_{n+1})
\]
if there are at least two integers $j=j_1,j_2$ such that
$s_j<d_j$,
and homogeneous of degree
\[
  n\, d_1\ldots d_{n+1}/d_{j_0}
\]
if there exists $j_0$ such that
$s_{j_0} < d_{j_0}$ and $s_j=d_j$ for all $j \neq j_0$.
\end{corollary}

This is the homogeneity property of the reduced resultant 
that particularizes  to give the degree of
$\Res(\flat F,\flat G)$ in Example~\ref{ex:toy}.


\begin{proof}
The grading of $\AZ$ we are considering is that of
Proposition~\ref{res:quasihom.b}, with $k=0$;
%the ring $\AZ$ is graded by \eqref{eq:gradingres2}, with $k=0$,
thus for all $j=1,\ldots,n+1$ the coefficients of $F_{j,l}$ all have weight
$l$, for $l=0,\ldots,d_j$.
Then we know by Proposition~\ref{res:quasihom.b} that the resultant of 
$F_1,\ldots,F_{n+1}$ is homogeneous of degree
$n\, d_1\cdots d_{n+1}$,
and by the same argument the resultant of $G_1,\ldots, G_{n+1}$
is homogeneous of degree
$n\, s_1\cdots s_{n+1}$.
Therefore, we deduce from Theorem~\ref{T:red-Zgrad} that the reduced
resultant of $H_1,\ldots,H_{n+1}$ is homogeneous,
of degree
\[
  n\, d_1\cdots d_{n+1}
  - n\, s_1\cdots s_{n+1}
\]
if $s_j<d_j$ for two distinct indices $j=j_1,j_2$,
and of degree
\[
  \frac
  {n\, d_1\cdots d_{n+1}
    - n\, s_1\cdots s_{n+1}}
  {d_{j_0}-s_{j_0}}
  = n\,
  \frac {d_1\cdots d_{n+1}}{d_{j_0}} \,
  \frac {d_{j_0}-s_{j_0}} {d_{j_0}-s_{j_0}}
\]
if $s_j=d_j$ for all $j\neq j_0$ and $s_{j_0}<d_{j_0}$.
\end{proof}


\section{Reduced discriminant and Salmon formula}
\label{S:redDisc}

In this Section we give a rigorous proof of formula
\taylordisc.\ This is done by introducing the concept of reduced
discriminant. 
We begin with a quick recap on the ordinary discriminant of a
hypersurface, following \cite[\S 4]{BJ14}; see also \cite{demazure}
and \cite[Chapter 13, \S D]{GKZ-16}.

\subsection{Discriminant of a homogeneous polynomial}

\paragraph{}
\label{p:notation-disc}
Let $d$ be a positive integer, and
consider the generic homogeneous degree  $d$ polynomial
$F=\sum_{|\balpha|=d}U_{\alpha}\bX^\balpha$ in $n+1$ indeterminates
$\bX=(X_0,\ldots,X_n)$.
We set $\AZ=\Z[U_{\balpha}] _{|\balpha|=d}$.
For all $i=0,\ldots,n$ we let $\d i$ denote derivation with respect to
the indeterminate $X_i$.

\begin{definition}\label{def:disc}
There is a unique element $\Disc_d (F) \in \AZ$ 
(often simply denoted by $\Disc (F)$) such that
\begin{equation}
\label{def:disc:eq}
d^{a(n,d)} \Disc_d(F) = \Res \bigl( \d 0 F,\ldots, \d n F \bigr)
\end{equation}
in $\AZ{}$, where $a(n,d) = \frac {(d-1)^{n+1}-(-1)^{n+1}} d \in
\Z$. It is homogeneous of degree $(n+1)(d-1)^n$ with respect to the
coefficients of the polynomial $F$, \ie with respect to the
indeterminates
$U_{\balpha}$, $|\balpha|=d$. 

For a homogeneous degree $d$ polynomial $f \in \k[\bX]$, we
define the \emph{discriminant} $\Disc(f) \in \k$ of $f$
as the specialization $\sigma (\Disc (F)) \in \k$, where $\sigma: \AZ \to \k$
is the unique specialization morphism mapping $F$ to $f$.
\end{definition}

We emphasize that the factor $d^{a(n,d)}$
in Equation~\eqref{def:disc:eq} is here to make the discriminant a
universal object (i.e., to make it behave well under specialization) which yields the expected smoothness criterion. An alternative way of defining the discriminant is to use
Formula~\eqref{disc-inter2} below. Either way there is an annoying
parasitic factor. The issue comes from the fact that, while the
resultant characterizes the existence of a non-trivial common zero
in $\P^n$ for $n+1$ polynomials, the wish for the discriminant is that
it will characterize the existence of a non-trivial common zero for
the $n+2$ polynomials $F, \d 0 F,\d 1 F,\ldots, \d {n} F$ which are
linked by the Euler Formula. The next result tells us that with
Definition~\ref{def:disc}, the discriminant grants our wish.

\begin{proposition}\label{prop:discInertie} The ideal of inertia forms
\[
  (\d 0 F,\d 1 F,\ldots, \d {n} F,F) : (X_0,\ldots,X_n)^\infty
\]
is a prime and principal ideal in $\AZ$.
It is generated by the discriminant $\Disc (F)$, which is therefore an
irreducible polynomial in $\AZ$.
\end{proposition}

In fact, what we really want is that the (non-)vanishing of the
discriminant characterizes smoothness. By the Jacobian criterion for
smoothness, this is equivalent to the non-existence of a common root
$F, \d 0 F,\d 1 F,\ldots, \d {n} F$. Thus,
Proposition~\ref{prop:discInertie} gives the following.

\begin{theorem}[smoothness criterion]
\label{t:sm-crit}
Suppose $\k$ is an algebraically closed field, and consider a degree
$d$ homogeneous polynomial $f \in \k[\bX]$. The following are
equivalent:
\begin{mycpctenum}
\item the hypersurface $\V(f) \subset \P^n _\k$ is smooth;
\item $\Disc (f) \neq 0$.
\end{mycpctenum}
\end{theorem}

The following formula gives an alternative way of defining the
discriminant. This is the path we shall follow to define the reduced
discriminant. As we shall see, however, there will be some additional
technical difficulty to overcome, which did not occur when passing
from the ordinary resultant to its reduced form either.


\begin{proposition}
\label{p:ident-disc}
Let $\bar F$ be the polynomial
$F(0,X_1,\ldots,X_{n}) \in \AZ{}[X_1,\ldots,X_{n}]$.
We have the following identity in $\AZ$:
\begin{equation}
\label{disc-inter2}
\Res \bigl( \d 1 F,\ldots, \d {n}F,F \bigr)
= \Disc(F)
\cdot \Disc(\bar F).
\end{equation}
\end{proposition}

The polynomial $\bar F$
is the equation of the hypersurface in $\P^{n-1}$ cut out by $\V(F)$
on the hyperplane $\V(X_0)\subset \P^{n}$, of which we think as the
hyperplane at infinity.
If $\k$ is an algebraically closed field and
$f \in \k[\bX]$ is a degree $d$ homogeneous polynomial,
then, 
by Theorem~\ref{t:sm-crit}, the vanishing of 
$\Disc(\bar f)$ is equivalent to the hyperplane section at infinity
$\V(f) \cap \V(X_0)$ being singular.
For a general $f$ such that $\Disc(\bar f)=0$, the hypersurface $\V(f)$
is non-singular and tangent to the hyperplane $\V(X_0)$.

\begin{proof}[Proof of Proposition~\ref{p:ident-disc}]
We shall prove the following identity in $\AZ$:
\begin{equation}
\label{disc-inter}
d^{(d-1)^n} \Res \bigl( \d 1 F,\ldots, \d {n}F,F \bigr)
= \Res \bigl(\d 0 F,\ldots, \d {n} F \bigr) 
\cdot \Res\bigl(\d 1 \bar F,\ldots, \d {n} \bar F\bigr).
\end{equation}
We claim that it is equivalent to Formula~\eqref{disc-inter2}.
To see why, first note that at the right-hand-side of
Display~\eqref{disc-inter}, 
the first (respectively second) factor is the resultant of $n+1$
(respectively $n$) polynomials in
$n+1$ (respectively $n$) indeterminates.
Since $a(n,d)+a(n-1,d)=(d-1)^n$, it follows from
Formula~\eqref{def:disc:eq} that the identities 
\eqref{disc-inter} and \eqref{disc-inter2} are indeed equivalent.

Now, the identity \eqref{disc-inter} may be derived from the Euler
Formula, as follows. The latter formula says that
$d\cdot F$ is congruent to $X_0\,\d 0 F$ modulo the ideal
$(\d 1 F,\ldots, \d n F)$, hence
\begin{equation}
\label{euler1}
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, d\cdot F \bigr)
  = \Res \bigl( \d 1 F,\ldots, \d {n}F,\, X_0\,\d 0 F \bigr)
\end{equation}
by \cite[\S 5.9, Transformations élémentaires]{J91}.
The left-hand-side of \eqref{euler1} equals that of \eqref{disc-inter}
by the elementary homogeneity properties of the resultant,
see Theorem~\ref{T:res}. Its
right-hand-side, on the other hand, equals
\begin{equation*}
%\label{euler2}
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, X_0 \bigr)
  \cdot
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, \d 0 F \bigr)
\end{equation*}
by multiplicativity of the resultant, see
\cite[\S 5.7]{J91}.
Eventually,
\begin{equation*}
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, X_0 \bigr)
  = (-1)^{n(d-1)^n}
  \Res \bigl( \restr {\d 1 F} {X_0=0},\ldots,
  \restr {\d {n}F} {X_0=0} \bigr)
\end{equation*}
by \cite[(5.13.5)]{J91}\footnote
{the $(-1)^{n(d-1)^n}$ factor is due to the fact that we need to
exchange the roles of $X_0$ and $X_n$, which is not indifferent since
by definition the resultant is normalized by imposing
$\Res(X_0^{d_0},\ldots,X_n^{d_n})=1$, see right after
Theorem~\ref{T:res}.

To work out the claimed identity, one may first perform a base change
by exchanging 
$X_0$ and $X_n$ which, by \cite[(5.13.1)]{J91}, gives
\[
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, X_0 \bigr)
  = (-1)^{(d-1)^n} \Res \bigl(
  \d{1}F(X_n,X_1,\ldots, X_{n-1}, X_0), \,\ldots, \ X_n \bigr);
\]
then, apply \cite[(5.13.5)]{J91} to the resultant on the
right-hand-side, and eventually perform another base change to go from
$(X_1,\ldots,X_{n-1},X_0)$ to $(X_0, X_1,\ldots,X_{n-1})$, which
introduces the additional factor
$(-1)^{(n-1)(d-1)^n}$, hence in total the factor
$(-1)^{n(d-1)^n}$ indeed.

An easier way to get the correct sign in general is to consider the
normalizing condition, once one knows that there exists $c \in \Z$
such that 
\[
  \Res_{d_1,\ldots,d_n,1} (F_1,\ldots,F_n, X_0)
  = c\,
  \Res_{d_1,\ldots,d_n} (\restr {F_1} {X_0=0},\ldots, \restr {F_n} {X_0=0}).
\]
Specializing $F_1,\ldots,F_n$ to $X_1^{d_1},\ldots,X_n^{d_n}$
respectively, one gets
\[
  \Res_{d_1,\ldots,d_n,1} (X_1^{d_1},\ldots,X_n^{d_n}, X_0)
  = c\,
  \Res_{d_1,\ldots,d_n} (X_1^{d_1},\ldots,X_n^{d_n}),
\]
where the left-hand-side equals
$(-1)^{nd_1\cdots d_n}$ by \cite[\S 5.8]{J91}, and the right-hand-side
equals $c$.
}, and
\begin{equation*}
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, \d 0 F \bigr)
  = (-1)^{n(d-1)^{n+1}} \Res \bigl( \d 0 F,\, \d 1 F,\ldots, \d {n}F \bigr)
\end{equation*}
by \cite[\S 5.8, Effet d'une permutation des polynômes]{J91}.
The upshot is that
\[
  \Res \bigl( \d 1 F,\ldots, \d {n}F,\, X_0\,\d 0 F \bigr)
  = (-1)^{nd(d-1)^n}\,
  \Res \bigl(\d 0 F,\ldots, \d {n} F \bigr) 
  \cdot \Res\bigl(\d 1 \bar F,\ldots, \d {n} \bar F\bigr),
\]
which gives the result since $d(d-1)$ is always even.
\end{proof}


Similarly to the resultant, the
discriminant is homogeneous under the two gradings of the
coefficient ring $\AZ$ introduced in Propositions \ref{res:quasihom.a}
and \ref{res:quasihom.b}.

\begin{proposition}
\label{par:weightdisc}
Let $k$ be an integer in $\intint 0 {n}$.
\subparagraph{}
\label{par:weightdisc.a}
In the grading of $\AZ$ defined by $\weight(U_\balpha)=\alpha_k$, 
the discriminant $\Disc (F)$ is homogeneous of degree $d(d-1)^{n}$.
\subparagraph{}
\label{par:weightdisc.b}
In the grading of $\AZ$ defined by $\weight(U_\balpha)=d-\alpha_k$, 
the discriminant $\Disc (F)$ is homogeneous of degree $nd(d-1)^{n}$.
\end{proposition}


One may use \ref{par:weightdisc.a}
to compute the degree of the dual to a smooth
hypersurface in $\P^{n+1}$, 
see Paragraph \ref{p:deg-dual}.


\begin{proof}
The idea is to consider \eqref{def:disc:eq} and the
corresponding weight properties of the resultant.
We may assume $k\neq 0$, for otherwise we may write a formula
analogous to \eqref{disc-inter2} with respect to an
indeterminate other than $X_0$ in order to reduce to this case.

First consider the grading of \ref{par:weightdisc.a}.
For $j\neq k$ the coefficient of $\d{j}F$ in $\bX^\balpha$ has weight
$\alpha_k$,
whereas for $j=k$ the coefficient of $\d{k}F$ in $\bX^\balpha$ has weight
$\alpha_k+1$. We may thus apply Corollary~\ref{p:further-wt}
to the homogeneity property \ref{res:quasihom.a},
with
$r_k=1$ and $r_j=0$ for all $j\neq k$, which gives that
$\Res \bigl( \d{0}F,\ldots,\d{n}F \bigr)$ is homogeneous of degree
\[
  (d-1)^{n+1} + (d-1)^{n}.
\]
Using \eqref{def:disc:eq}, this gives \ref{par:weightdisc.a}.

Similarly, for the grading of \ref{par:weightdisc.b}:
for $j\neq k$ the coefficient of $\d{j}F$ in $\bX^\balpha$ has weight
$d-\alpha_k=(d-1)-\alpha_k+1$,
whereas for $j=k$ the coefficient of $\d{k}F$ in $\bX^\balpha$ has weight
$d-(\alpha_k+1)=(d-1)-\alpha_k$.
We thus apply Corollary~\ref{p:further-wt}
to the homogeneity property \ref{res:quasihom.b},
with $r_j=1$ for $j\neq
k$ and $r_k=0$, which gives
 that
$\Res \bigl( \d{0}F,\ldots,\d{n}F \bigr)$ is homogeneous of degree
\[
  n(d-1)^{n+1} + n(d-1)^{n}.
\]
Again this gives the wanted result by \eqref{def:disc:eq}.
\end{proof}

In turn, one may reproduce the argument given in \ref{p:further-wt} to
deduce further weight properties from the two latter results and the
standard homogeneity property of the discriminant stated in
Definition~\ref{def:disc}. 

\begin{corollary}
\label{c:further-wt-disc}
Assume that the discriminant $\Disc_d \in \AZ$
is homogeneous of degree
$\delta$ for the grading on $\AZ$ defined by
$\weight(U_{\balpha}) = w_{\balpha}$.
Let $r \in \Z$.
For the new grading on $\AZ$
defined by $\weight(U_{\balpha}) = w_{\balpha}+r$,
the discriminant $\Disc_d$
is homogeneous of degree
\[
\delta + r (n+1)(d-1)^n.
\]
\end{corollary}



\subsection{The reduced discriminant}
\label{s:redDisc}

\paragraph{}
\label{p:setup-redDisc}
We write the generic homogeneous degree  $d$ polynomial as
\[
F %(x_0,\ldots,x_n)
=X_0^d F_0
% (x_1,\ldots,x_{n-1})
+\cdots
+X_0^{d-s} F_s
+ \cdots + F_d
\]
where each $F_k$ is homogeneous of degree $k$ in the indeterminates
$X_1,\ldots,X_{n}$. 
Given an integer $s \in \intint{2}{d-1}$,
we consider the truncation $H$ of $F$ at order $d-s$ with respect to
$X_0$, defined as in Paragraph~\ref{par:redresnotation},
and set $G$ as in Paragraph~\ref{p:G_j}; thus,
\begin{alignat*}{2}
H &= && X_0^{d-s}F_s
+X_0^{d-s-1}F_{s+1}+\cdots+F_d,
\\
G &= X_0^{s}F_0+X_0^{s-1}F_1+\cdots+&&F_s.
\end{alignat*}
The truncation $H$ is the generic degree $d$ polynomial with a
multiplicity $s$ zero at the point $(1\!:\!0\!:\!\ldots\!:\!0)$.
The wish for the reduced discriminant is that it is a polynomial in
the coefficients of $H$, the vanishing of which characterizes the
existence of an additional singular non-trivial zero of $H$.

The polynomial $H$ is homogeneous of degree $d$, and
has \valuation{} $s$ in $X_1,\ldots,X_n$
(recall Definition \ref{d:order}).
Moreover, its partial
derivatives with respect to the indeterminates $X_1,\ldots,X_n$ all
have degree $d-1$, and \valuation{} $s-1$ in $X_1,\ldots,X_n$.
Therefore, the reduced resultant 
\[\redRes(\d 1 H,\ldots,\d n H, H)
= \redRes _{d-1,\ldots,d-1,d} ^{s-1,\ldots,s-1,s} 
(\d 1 H,\ldots,\d n H, H)
\]
is well defined. 

\begin{proposition}
\label{p:div-redRes}
With the above notation, the discriminants $\Disc(F_s)$ and
$\Disc(F_d)$ both divide the reduced resultant $\redRes(\d 1
H,\ldots,\d n H, H)$.
\end{proposition}

\begin{proof} 
Both discriminants $\Disc(F_s)$ and $\Disc(F_d)$ are 
irreducible as elements of $\AZ{}$,
and therefore coprime because they do not depend on the same
coefficients of $F$.
To prove the proposition, it thus suffices to prove
that the vanishing of $\Disc(F_s)$ or $\Disc(F_d)$
implies the vanishing of the reduced resultant.
This follows from \ref{p:geominterp-redres}, as we shall now explain.

The vanishing of $\Disc(F_d)$ at $f$ (a specialization of $F$ with
coefficients in an algebraically closed field $\k$)
implies the existence of a common root at infinity ($x_0=0$) of the
polynomials $h, \partial_1h,\ldots,\partial_nh$
(with $h$ the specialization of $H$ corresponding to $f$).
Indeed, if $\Disc(F_d)$ vanishes at $f$, then by
Theorem \ref{t:sm-crit} there exists a non-trivial zero
$\flat x \in \k^n$ of $f_d, \d1 f_d, \ldots \d n f_d$,
and then $(0, \flat x) \in \k^{n+1}$ is a non-trivial zero of
$h, \d1 h, \ldots, \d n h$, hence the reduced resultant vanishes at
$f$ by (a) of \ref{p:geominterp-redres}.

Similarly,
the vanishing of $\Disc(F_s)$ at $f$ implies the existence of a common
non-trivial zero of $h, \d1 h, \ldots, \d n h$
infinitely near the point $p_0 = (1\!:\!0\!:\!\ldots\!:\!0)$:
indeed, $f_s, \d 1 f_s,\ldots, \d n f_s$ define the respective tangent
cones at $p_0$ of the hypersurfaces $V(h), V(\d 1 h), \ldots, V(\d n h)$,
and the vanishing of $\Disc(F_s)$ at $f$ implies the existence of a
non-trivial zero 
$\flat x \in \k^n$ of $f_s, \d1 f_s, \ldots \d n f_s$.
Thus, by (b) of \ref{p:geominterp-redres}, the reduced resultant
vanishes at $f$ if $\Disc(F_s)$ vanishes at $f$.
\end{proof}

Alternatively, this proposition can be proved by means of
inertia forms, as follows.
By Theorem \ref{thm:redres}, the reduced
resultant $\redRes(\d 1 H,\ldots, \d {n}H,H)$ belongs to the ideal of
inertia forms $(\d 1 H,\ldots,
\d {n}H,H):(X_1,\ldots,X_n)^\infty$. Therefore, for all integer
$i=1,\ldots,n$, there exists an integer $N_i$ such that
\begin{equation}\label{eq:redresInertie}
  X_i ^{N_i} \redRes(\d 1 H,\ldots, \d {n}H,H)
  \in (\d 1 H,\ldots, \d {n}H,H);
\end{equation}
specializing the variable $X_0$ to $0$ in \eqref{eq:redresInertie}, we
get that
\[
  X_i ^{N_i} 
\redRes(\d 1 H,\ldots, \d {n}H,H) \in (\d 1 F_d,\ldots, \d {n}
F_d,F_d).
\]
It follows that
$\redRes(\d 1 H,\ldots, \d {n}H,H)$ belongs to the ideal of inertia
forms
$(\d 1 F_d,\ldots,\d n F_d, F_d) :(X_1,\ldots,X_n)^\infty$.
By Proposition \ref{prop:discInertie}, this ideal is generated by the
discriminant of the polynomial $F_d$, hence $\Disc(F_d)$
divides $\redRes(\d 1 H,\ldots,\d n H, H)$. A similar argument, albeit
slightly more technical, can be used to show that $\Disc(F_s)$ divides
$\redRes(\d 1 H,\ldots,\d n H, H)$: see \cite[Lemme I.1.3]{OM88}.


\bigskip
In the notation of \ref{p:ident-disc}, 
$F_d=\bar F$ and $F_s = \bar G$. 
Observe that $F_d$ and $F_s$ are generic homogeneous polynomials of
degrees $d$ and $k$ respectively, in the indeterminates $(X_1,\ldots,X_n)$.
Proposition~\ref{p:div-redRes} then leads to the following definition.

\begin{definition}
\label{defn:reddisc}
The \emph{reduced discriminant} of $F$ with respect to the truncation
at order $d-s$ for the indeterminate $X_0$, denoted by
$\redDisc^s_{d}(H)$, or simply $\redDisc(H)$, is defined by the
equality
\begin{equation}
\label{eq:defreddisc}
\Disc(F_d)\,\Disc(F_s)
\redDisc (H)
= \redRes \bigl( \d 1 H,\ldots, \d {n}H, H \bigr)
\in \AZ.
\end{equation}
\vspace{-\belowdisplayskip}
\end{definition}

\noindent
For a degree $d$ polynomial $h\in \k[\bX]$ with a singularity of order
$s$ at the origin,
$\redDisc_d^s(h)$ is defined as the specialization of
$\redDisc_d^s(H)$
with respect to the unique specialization $\AZ\to \k$ mapping $H$ to
$h$.

Definition~\ref{defn:reddisc} implies that $\redDisc(H)$ is a primitive 
polynomial in $\AZ{}$ (\ie the greatest common divisor of its
coefficients equals $1$),
because $\redRes(\d 1 H,\ldots, \d {n}H, H)$ is primitive
by \cite[Proposition 4.24]{BJ14}.

The identity \eqref{eq:defreddisc} should be compared to 
\eqref{disc-inter2}. Beware that the reduced discriminant is not
merely the reduced resultant of all the partial derivatives, because
of the factor $\Disc(F_s)$ in \eqref{eq:defreddisc}.
The factor $\Disc(F_d)$ is an artefact of
our definition by considering
$\redRes \bigl( \d 1 H,\ldots, \d {n}H, H \bigr)$
and not plainly $\redRes \bigl( \d{0}H, \d 1 H,\ldots, \d {n}H
\bigr)$, in order to define the
reduced discriminant as a primitive polynomial with integer
coefficients without dealing with possible constant factors, similar
to $d^{a(n,d)}$ in \eqref{def:disc:eq}.
The factor $\Disc(F_s)$ on the other hand is geometrically meaningful, 
as we will see in
\ref{p:geominterp-reddisc} below.


\bigskip
According to \eqref{def:disc:eq}, the classical discriminant of a
homogeneous polynomial can be computed from the resultant of all its
partial derivatives, up to the extraneous integer factor
$d^{a(n,d)}$. It turns out that a similar formula holds for the
reduced discriminant.

\begin{proposition}
\label{p:demazure-reddisc}
The following identity in $\AZ{}$ holds:
\begin{equation}
\label{eq:reddisc-demazure}
d^{a(n,d)-(s-1)^n} \Disc(F_s)\redDisc(H)
=\redRes(\partial_0 H,\ldots,\partial_n H).	
\end{equation}
\end{proposition}

\begin{proof}
To prove this formula, we consider the reduced resultant 
$\mathcal{R}:=\redRes(\partial_1 H,\ldots,\partial_n H, dH)$. First,   
from the homogeneity property (see Theorem \ref{thm:redres}), we have
\begin{equation*}
\label{eq:redDis-Dem1}
\mathcal{R}:=d^{(d-1)^n-(s-1)^n} \redRes(\partial_1 H,\ldots,\partial_n H, H).	
\end{equation*}
Next, the Euler Identity gives $\mathcal{R}:=\redRes(\partial_1 H,\ldots,\partial_n H, \sum_{i=0}^n X_i\partial_iH)$,
and we claim that 
\begin{align}
	\label{eq:redDisc-Dem2}
	\mathcal{R} &= \redRes(\partial_1 H,\ldots,\partial_n H, X_0\partial_0H) \\
	\label{eq:redDisc-Dem3}
				&= (-1)^{n(d-1)^n} \Res(\partial_1F_d,\ldots,\partial_nF_d)\redRes(\partial_1 H,\ldots,\partial_n H, \partial_0 H)
\end{align}
(observe that $\partial_0H$ has degree $d-1$ and \valuation{} $s$
in $X_1,\ldots,X_n$, and
$\restr H {X_0=0} = F_d$). 
We conclude the proof of \eqref{eq:reddisc-demazure} before justifying
the two above equalities. The Zariski formula together with the property of resultants under permutation of the polynomials \cite[\S 5.8]{J91} yields the equality:
\[
  \redRes(\partial_1 H,\ldots,\partial_n H, \partial_0 H)
  =(-1)^{n(d-1)^{n+1}-ns(s-1)^{n}}
  \redRes(\partial_0 H,\ldots,\partial_n H).
\]
In addition, $\Res(\partial_1F_d,\ldots,\partial_nF_d)=d^{a(n-1,d)}\Disc(F_d)$, so putting everything together, including \eqref{eq:defreddisc}, we deduce that
$$d^{(d-1)^n-(s-1)^n-a(n-1,d)} \Disc(F_s)\redDisc(H)=(-1)^N \redRes(\partial_0 H,\ldots,\partial_n H),$$
where $N=n(d-1)^n+n(d-1)^{n+1}-n(s-1)^ns=nd(d-1)^n-n(s-1)^ns$.
Now, $N$ is an even integer, and 
$(d-1)^n-a(n-1,d) = a(n,d)$, hence the claimed formula.

To justify \eqref{eq:redDisc-Dem2}, we prove the following invariance property of the reduced resultant under some elementary transformations. Let $F_1,\ldots,F_{n+1}$ be generic polynomials of degree $d-1,\ldots,d-1,d$ respectively, as well as generic linear forms $L_1,\ldots,L_n$ in the variables $X_1,\ldots,X_n$. Then, from the definition of the reduced resultant as a generator of the ideal of inertia forms in the generic setting, we deduce that
$$\redRes_{d-1,\ldots,d-1,d}^{s-1,\ldots,s-1,s}(H_1,\ldots,H_{n+1})
\text{ divides }
\redRes_{d-1,\ldots,d-1,d}^{s-1,\ldots,s-1,s}(H_1,\ldots,H_{n+1}+\sum_{i=1}^n L_iH_i).
$$ 
We notice that this divisibility property remains valid under any
specialization, in particular under the specialization sending
$F_{n+1}$ to $F_{n+1}-\sum_{i=1}^nL_i F_i$, and leaving
$F_1,\ldots,F_n$ invariant. This implies that the above divisibility
property also holds in the other direction, hence these two reduced
resultant are equal, up to sign. Applying Zariski formula and the invariance of the resultant under elementary transformations \cite[\S 5.9]{J91}, we deduce that this sign equals 1.   


The equality \eqref{eq:redDisc-Dem3}, on the other hand, is a consequence of the following multiplicativity property of the reduced resultant:
\begin{multline}
\redRes_{d_1,\ldots,d_{n+1}+1}^{s_1,\ldots,s_{n+1}}(H_1,\ldots,H_n,X_0H_{n+1}) \\
= (-1)^{d_1\cdots d_n}\Res(\bar{F_1},\ldots,\bar{F_n}) \cdot \redRes_{d_1,\ldots,d_{n+1}}^{s_1,\ldots,s_{n+1}}(H_1,\ldots,H_n,H_{n+1}),
\end{multline}
which follows from the Zariski formula. Indeed, let $F_1,\ldots,F_{n+1}$
be generic polynomials as above, and denote by $H_i$ and $G_i$ their
decompositions corresponding to the truncation at order
$d_i-s_i$ for all $i$. On the one hand, we have (observe that
$F_{n+1}$ and $X_0F_{n+1}$ have the same ``$G$'', namely $G_{n+1}$):
\begin{multline*}
\Res(F_1,\ldots,F_n,X_0F_{n+1})=\Res(G_1,\ldots,G_n,G_{n+1})\redRes(H_1,\ldots,H_{n},X_0H_{n+1})\\ 
 + \text{ terms of higher weight.}	
\end{multline*}
On the other hand, by properties of the classical resultant,
$$\Res(F_1,\ldots,F_n,X_0F_{n+1})=(-1)^{d_1\ldots,d_n}\Res(\bar{F_1},\ldots,\bar{F_n})\Res(F_1,\ldots,F_n,F_{n+1}),$$
hence, by the Zariski formula,
\begin{multline*}
\Res(F_1,\ldots,F_n,X_0F_{n+1})= \\
(-1)^{d_1\ldots,d_n}\Res(\bar{F_1},\ldots,\bar{F_n})\Res(G_1,\ldots,G_{n+1})\redRes(H_1,\ldots,H_{n+1}) + \text{ terms of higher weight}.
\end{multline*}
The comparison of the two above expressions of
$\Res(F_1,\ldots,F_n,X_0F_{n+1})$ yields the expected equality.
\end{proof}

 

\paragraph{Vanishing of the reduced discriminant}
\label{p:geominterp-reddisc}
By definition of the truncation $H$,
the generic hypersurface $\V(H) \subset \P^n$ has 
an ordinary $s$-fold point at the origin $(1\!:\!0\!:\!\ldots\!:\!0)$. 
By Paragraph~\ref{p:geominterp-redres},
% and \ref{defn:reddisc},
the vanishing of
$\redRes \bigl( \d 1 h,\ldots, \d {n}h, h \bigr)$ for some
specialization $h$ of $H$
in an algebraically closed field $\k$
%the product $\Disc(F_d)\cdot \Disc(F_s)\cdot \redDisc(H)$
corresponds to one of the two following properties: 
\begin{compactenum}[(a)]
\item the existence of a common zero for the
  polynomials $\d 1 h,\ldots,\d n h,h$ which is not the origin;
\item the existence of a common zero for the polynomials $\d 1 f_s,
  \ldots, \d n f_s, f_s$, equivalently a common root for the
  polynomials $\d 1 f_s, \ldots, \d n f_s$ by Euler Identity,
  assuming for simplicity that the degree $d$ is non-zero in $\k$.
\end{compactenum}

Property (b) is equivalent to the vanishing of $\Disc(f_s)$,
\ie to the tangent cone of the hypersurface
$\V(h)$ at the origin being a cone over a
singular degree $s$ hypersurface
(with the convention that a hypersurface of degree $s'>s$ is a
singular degree $s$ hypersurface); in other words, in the blow-up of
$\V(h)$ at the origin, the exceptional divisor is singular.
This is equivalent to the singularity of $V(h)$ at the origin being
worse than an ordinary $s$-fold point, but does not imply that the
blow-up of $V(h)$ is singular, see Example \ref{ex:worse}
below.

Property (a) is implied by the vanishing of $\Disc(f_d)$,
as we have seen in the proof of Proposition~\ref{p:div-redRes}.
The latter condition is equivalent to the
hypersurface $\V(h)$ being tangent to the hyperplane at infinity
$\V(X_0)$. 

In Definition~\ref{defn:reddisc} we discard the two factors
$\Disc(F_s)$ and $\Disc(F_d)$; the upshot is that the vanishing of the
reduced discriminant $\redDisc(H)$ defines
an (irreducible\footnote
{the proof of the irreducibility of the reduced
discriminant will appear in
\cite{BD2}, but this property also follows from the theory of toric
discriminants (see \cite[Chapter 9]{GKZ-16}), of which the reduced
discriminants are particular instances.
% \ref{com:future}.
})
divisor which has as a
dense subset the locus of those hypersurfaces $\V(h)$
that have a singularity off the origin.
This implies, since smoothness is an open property, that if
$\redDisc(H)$ vanishes at $h$, then
the proper transform\footnote
{here we take the following slightly abusive definition for the proper
transform: let $\epsilon: \tilde \P^n \to \P^n$ be the blow-up at the
origin, with exceptional divisor $E$;
the \emph{proper transform} of $V(h)$ is the divisor
$\epsilon^* V(h)-sE$.
If $V(h)$ has an ordinary $(s+1)$-fold at the origin, its genuine
proper transform is $\hat V(h) = \epsilon^* V(h)-(s+1)E$, which is
smooth along $E$, whereas its proper transform in our sense is
$\hat V(h)+E$, which is singular along $E$.
}
of $V(h)$ in the blow-up of the origin is
singular,
in other words $V(h)$ has an additional singularity, possibly
infinitely near, besides its $s$-fold point at the origin.
In fact the converse holds as well, as we shall see in \cite{BD2}.
Thus, $\redDisc(H)$ vanishes at $h$ if and only $V(h)$ has an
additional singularity, possibly infinitely near.

Note that we make a difference between having a singularity worse than
an ordinary $s$-fold point and having an additional singularity
infinitely near the ordinary $s$-fold point, see the following example
and \ref{p:milnor} below for more details.

\begin{example}
\label{ex:worse}
Set $n=2$  and $s=2$. In this case, $\Disc(F_2)$ vanishes at $h$ if
and only if $f_2$ is a square, equivalently, $h$ may be written as
\[
  h = X_0^{d-2}\, X^2 + X_0^{d-3}\, \bigl(a_3 Y^3
  + a_2 X Y^2
  + a_1 X^2 Y
  + a_0 X^3\bigr)
  +\, \cdots
\]
after a suitable change of coordinates
$(X,Y) = \phi(X_1,X_2)$.
Let $\epsilon: \tilde \P^2 \to \P^2$ be the blow-up at the
origin.
The relevant place to study the proper transform of $V(h)$
over the origin $(1\!:\!0\!:\!0) \in \P^2$ is the
affine plane with coordinates $(U,Y)$ in $\tilde \P^2$ which dominates
the affine plane $(X_0=1)$ in $\P^2$, and such that
$\epsilon^*(X,Y) = (UY, Y)$.
In this affine chart, the pull-back $\epsilon^* h$ is given by
\[
  U^2Y^2 + \bigl(a_3 Y^3
  + a_2 UY^3
  + a_1 U^2 Y^3
  + a_0 U^3Y^3\bigr)
  +\, \cdots
\]
and the proper transform of $V(h)$ is defined by the equation
obtained by factoring out $Y^2$ from $\epsilon^* h$, \ie
\[
  U^2 + \bigl(a_3 Y
  + a_2 UY
  + a_1 U^2 Y
  + a_0 U^3Y\bigr)
  +\, \cdots
\]
This shows that the proper transform of $V(h)$ is singular at some
point lying on the
exceptional divisor of $\epsilon$
(defined by $Y=0$ in this affine chart) if and
only if $a_3=0$.

The generic $h$ such that $\Disc(F_2)$ vanishes defines a plane curve
with an ordinary cusp at the origin (local equation $x^2+y^3 = 0)$;
the proper transform of this curve in the blow-up at the origin is
smooth (and tangent to the exceptional divisor), hence
$\redDisc(H)$ does not vanish at $h$
even though $V(h)$ has a singularity worse than an ordinary double
point at the origin.
On the other hand,
the generic $h$ such that $V(h)$ has an additional singularity
infinitely near the origin
(which implies that $\redDisc(H)$ vanishes) defines a plane curve
with a tacnode at the origin (local equation $x^2+y^4=0$, two smooth
local branches tangent to each other); the proper transform of such a
curve has an ordinary double point located on the exceptional divisor.
\end{example}

\begin{remark}
In the reduced resultant situation, the condition that the $n+1$
hypersurfaces $\V(h_1),\ldots,\V(h_{n+1})$ have an infinitely near
additional intersection point is not divisorial,
\ie it does not correspond to an irreducible element factoring out of
$\redRes(H_1,\ldots,H_{n+1})$.
The reason is that this condition has codimension larger than one:
indeed it amounts to the $n+1$ leading terms 
$f_{1,s_1},\ldots,f_{n+1,s_{n+1}}$ having a non-trivial common zero,
in other words the $n+1$ corresponding hypersurfaces in $\P^{n-1}$
have non-trivial intersection: these are $n+1$ hypersurfaces in
$\P^{n-1}$, hence the condition has codimension larger than one.

In contrast, in the reduced discriminant situation the condition that
the hypersurface $\V(h)$ has a singularity worse than an ordinary
$s$-fold point is divisorial, as it corresponds to the vanishing of
$\Disc(F_s)$ at the leading term $f_s$ of $h$.
The vanishing of $\redDisc(H)$ at $h$ is not implied by the latter
condition, but by the stronger condition that $V(h)$ has an additional
singularity infinitely near its $s$-fold point.
\end{remark}


\paragraph{}
\label{p:milnor}
We may use the Milnor number
(see \cite[Section \tref{S:algebroid}]{02.edoardo}
for the definition) to give a precise meaning to the condition of
having a singlarity worse than an ordinary $s$-fold point.
Assume that $h$
defines a hypersurface with an isolated singularity at the origin, so
that its Milnor number at the origin $\mu_0(h)$ is well-defined.
If the singularity of $h$ at the origin is an ordinary $s$-fold point,
then $\mu_0(h)=(s-1)^n$, and condition (b)
in Paragraph~\ref{p:geominterp-reddisc} above
is equivalent to the condition that
$\mu_0(h)>(s-1)^n$ by \cite[Theorem~1]{FuTo04}.


\begin{lemma}
In the standard grading of $\AZ$,
given by $\weight(U_\balpha)=1$ for all $\balpha$,
the reduced discriminant $\redDisc_d^s$ is homogeneous of degree
\begin{equation}\label{eq:degreereddisc}
(n+1)\bigl[ (d-1)^n - (s-1)^n \bigr] - 2n(s-1)^{n-1}.
\end{equation}
\end{lemma}

\begin{proof}
This follows from the definition by a direct computation, since the
degrees of the other quantities in Display~\eqref{eq:defreddisc} are
known. It is arguably safer, however, to
carry this out explicitly.

The two plain discriminants $\Disc(F_d)$ and $\Disc(F_s)$ are
homogeneous of respective degrees
$n(d-1)^{n-1}$ and $n(s-1)^{n-1}$, see Definition~\ref{def:disc}.
Moreover, it follows from Theorem~\ref{thm:redres} that
\[
  \redRes _{d-1,\ldots,d-1,d} ^{s-1,\ldots,s-1,s}\, 
  (\d{1}H, \ldots, \d{n}H, H)
\]
is homogeneous of  degree
\[
  n\bigl( d(d-1)^{n-1} -s(s-1)^{n-1} \bigr)
  + \bigl( (d-1)^n - (s-1)^n \bigr).
\]
It thus follows from the equality in Display~\eqref{eq:defreddisc}
that $\redDisc(H)$ is homogeneous, of degree
\begin{multline*}
  \bigl[ nd(d-1)^{n-1} +(d-1)^n -n(d-1)^{n-1} \bigr]
  - \bigl[ ns(s-1)^{n-1} +(s-1)^n +n(s-1)^{n-1} \bigr]
  \\
  = (n+1)(d-1)^n
  -(s-1)^{n-1} \bigl((n+1)s+n-1\bigr),
\end{multline*}
and the result follows.
\end{proof}

\noindent
We now turn to the generalized weight properties of the reduced
discriminant. 

\begin{example}\label{ex:reddiscn=1}
As an illustrative example, we consider the case $n=1$ and set 
\[
F=\sum\nolimits_{i=0}^d U_iX_0^{d-i}X_1^i
=X_0^dF_0+X_0^{d-1}F_1+\cdots+X_0^{d-s}F_s+\cdots F_d,
\]
with $F_i=U_iX_1^i$ for all $i=0,\ldots,d$.  
We consider
\[
H= \sum\nolimits_{i=s}^d U_i X_0^{d-i} X_1^i
=\sum\nolimits_{i=s}^d X_0^{d-i}F_i
=X_1^s \bigl(
U_s X_0^{d-s} + U_{s+1} X_0 ^{d-s-1} X_1 + \cdots + U_d X_1 ^{d-s}
\bigr),
\]
the  truncation of $F$ at order $d-s>0$ with respect to $X_0$. 
Then, setting $H=X_1^{s}\cdot \flat H$ it is easy to check that
$\redDisc_d^s(H)=\pm \Disc(\flat H)$; it is therefore an irreducible
polynomial of degree $2(d-s-1)$ in the coefficients of $H$ (compare
with Formula~\eqref{eq:degreereddisc} for the degree).

Moreover, using the weight properties in
Proposition~\ref{par:weightdisc}, we can deduce weight properties of
$\redDisc(H)$. 
Suppose that $\AZ$ is graded with the rule
$\weight(U_i)=\max(0,i-s)$; then the reduced discriminant
$\redDisc_d^s(H)$ is homogeneous of degree
\begin{equation}
\label{reddisc-n1-a}
  (d-s)(d-s-1)
\end{equation}
by Proposition~\ref{par:weightdisc},
as $\flat H$ has degree $d-s$.
Similarly, if $\AZ$ is graded with the rule
$\weight(U_i)=d-i$ then the same conclusion holds
(note that $d-i = (d-s)-(i-s)$).

We can generalize this following Corollary~\ref{p:further-wt}.
Let $r$ be an integer and consider the grading of $\AZ$ defined by the
rule $\weight(U_i)=i-s+r$ if $i \geq s$, and $\weight(U_i)=0$ otherwise, 
then
$\redDisc_d^s(H)$ is homogeneous 
of degree $(d-s+2r)(d-s-1)$. In particular, if $r=s$,
\ie $\weight(U_i)=i$ if $i \geq s$ and $\weight(U_i)=0$ otherwise, we
get that $\redDisc_d^s(H)$ is homogeneous of degree
\begin{equation}\label{eq:redDiscn=1}
(d+s)(d-s-1)=d(d-1)-s(s+1).
\end{equation}
In fact, since $\redDisc_d^s(H)$ a polynomial in $U_s,\ldots,U_d$ only, 
the weights of $U_0,\ldots,U_{s-1}$ don't matter.
Similarly, in the grading of $\AZ$ is defined by the rule
$\weight(U_i)=d-i+r$ if $i \geq s$ and $\weight(U_i)=0$ otherwise,
$\redDisc_d^s(H)$ is homogeneous of degree $(d-s+2r)(d-s-1)$.
\end{example}


The following result is similar to Theorem~\ref{T:red-Zgrad}.
It is the key to the generalized Salmon formula for the discriminant.
\begin{theorem}[{\cite[Theorem 4.25]{BJ14}}]
\label{thm:valdisc}
Suppose that the ring $\AZ{}$ is graded by means of the Zariski
grading \ref{p:Zdeg},
\ie $\weight(U_\balpha)=\max(\alpha_0-d+s,0)$. Then $\Disc(F)$ has
\valuation{} $s(s-1)^{n}$, and its homogeneous part $D_0$ in this degree
satisfies the following equality in $\AZ$:
\begin{equation}
\label{leastdeg-disc}
D_0 \, \Disc(F_d)
= \Disc(G) 
\, \Disc (F_s) 
\, \redRes \bigl( \d{1}H,\ldots, \d{n}H, H
\bigr).
\end{equation}
%\negvcorr
\end{theorem}

Let us point out that the three elements $\Disc(F_d)$, $\Disc (F_s)$, and
$\redRes (\d 1H,\ldots, \d {n}H, H)$ 
have degree $0$ with respect to the Zariski grading, while
$\Disc(G)$ is homogeneous of degree $s(s-1)^n$ by
\ref{par:weightdisc.a};
% \eqref{disc-inter2} and \ref{res:quasihom};
note that $F_d$ and $F_s$ are
generic homogeneous polynomials of respective degrees $d$ and $s$ in
the indeterminates $(X_1,\ldots,X_n)$,
while $G$ is generic homogeneous of degree $s$ in $(X_0,\ldots,X_n)$.

\begin{remark}
\label{p:salmon-hist}
The only trace towards the reduced discriminant in Salmon's work
that we have found is in \cite[\S 117]{salmon-inv},
where he proves, in the above language, that for $s=2$, $\Disc(F)$ has
\valuation{} at least $2$.

He obtains this as a direct consequence of the fact that if $f$ is a
polynomial which is 
singular at a point $x$, then the tangent space of the discriminant
hypersurface $\V(\Disc)$ at $[f]$ contains the hyperplane of
polynomials vanishing at $x$.
Thus, for the polynomial
\[
  f =
  \sum _{a>1} F_a X_0^{d-a}
  + T\cdot \bigl( U_1'X_1+\cdots + U_n'X_n\bigr)\,
  X_0^{d-1},
\]
one finds that $\Disc(f)$ is divisible by $T^2$
(here, $F$ is as in \ref{p:notation-disc}
and \ref{p:setup-redDisc},
and $T,U_1',\ldots,U_n'$ are new indeterminates).
It follows that $\Disc(F)$ sits in the ideal
\[
  \bigl( U_{d,0,\ldots,0} \bigr)
  + \bigl(
  U_{d-1,1,\ldots,0},\,
  \ldots\,,\,
  U_{d-1,0,\ldots,1}
  \bigr)^2
  \subset \AZ,
\]
which means that it has \valuation{} at least $2$ with respect
to the Zariski grading for $s=2$.
\end{remark}

\begin{proof}[Proof of Theorem~\ref{thm:valdisc}]
The idea is to specialize Theorem~\ref{T:red-Zgrad}, part (a), and in
particular the formula
\[
  \bigl[ \Res(F_1,\ldots,F_{n+1}) \bigr] _{s_1s_2\cdots s_{n+1}}
  =
  \Res(G_1,\ldots,G_{n+1})\cdot \redRes(H_1,\ldots,H_{n+1}),
\]
to the discriminant situation, \ie
$F_1,\ldots,F_{n+1}$ specialize to $\d{1}F,\ldots, \d{n}F, F$
respectively,
and the $G_j$'s and $H_j$'s specialize according to the truncations
corresponding to $s_1,\ldots,s_{n+1}=s-1,\ldots,s-1,s$, as
indicated in Paragraph~\ref{p:setup-redDisc}.
Thus, we consider the following specializations:
\begin{align*}
  \Res(F_1,\ldots,F_{n+1})
  &\leadsto
    \Res (\d{1}F,\ldots, \d{n}F, F)
    % = \Disc(F) \, \Disc(\bar F)
  \\
  \Res(G_1,\ldots,G_{n+1})
  &\leadsto
    \Res (\d{1}G,\ldots, \d{n}G, G)
    % = \Disc(G) \, \Disc(\bar G)
  \\
  \redRes(H_1,\ldots,H_{n+1})
  &\leadsto
    \redRes (\d{1}H,\ldots, \d{n}H, H)
    % = \redDisc(H) \, \Disc(F_d) \, \Disc(F_s)
\end{align*}
On the other hand, we have
\begin{align}
  \label{BJ-F}
  \Res (\d{1}F,\ldots, \d{n}F, F)
  &= \Disc(F) \, \Disc(\bar F)
  \\
  \label{BJ-G}
  \Res (\d{1}G,\ldots, \d{n}G, G)
  &= \Disc(G) \, \Disc(\bar G)
\end{align}
by Proposition~\ref{p:ident-disc}. By definition,
$\bar F = F_d$ and $\bar G = G_s = F_s$,
and the result follows.
We refer to \cite{BJ14} for more details.
\end{proof}

The following corollary is the general form of Salmon's formula. As we
will see in the next section, Salmon's formula is a particular form of
the corollary in the case $s=2$.

\begin{corollary}
\label{cor:generalizedSalmonFormula}
In the Zariski grading of $\AZ{}$ as in Theorem \ref{thm:valdisc},
the discriminant $\Disc(F)$ has \valuation{} $s(s-1)^{n}$, and can be
written as 
\begin{equation}
\label{eq:generalizedSalmonFormula}
  \Disc(F)
  = \Disc(G) 
  \, \Disc (F_s)^2 
  \, \redDisc (H)
  +\bigl(\mathrm{terms \ of \ Zariski \  weight} > s(s-1)^n
\bigr).
\end{equation}
\end{corollary}
% \negvcorr

\begin{proof}
The only novelty with respect to the previous theorem is the
expression for $D_0$ (in the notation of Theorem~\ref{thm:valdisc})
in terms of the reduced discriminant. By
Definition~\ref{defn:reddisc}, one has
\[
  \redRes \bigl( \d 1 H,\ldots, \d {n}H, H \bigr)
  = \Disc(F_d)\,\Disc(F_s) \,
  \redDisc (H).
\]
Thus, Equation~\eqref{leastdeg-disc} writes
\begin{equation*}
D_0 \, \Disc(F_d)
= \Disc(G) 
\, \Disc (F_s) 
\,  \Disc(F_d)\,\Disc(F_s) \,
  \redDisc (H)
\end{equation*}
which gives
\begin{equation*}
D_0 
= \Disc(G) 
\, \Disc (F_s) ^2
  \redDisc (H)
\end{equation*}
as we wanted.
\end{proof}

We point out that, in the above,
the factor $\Disc (F_s)$ comes once from
Formula~\eqref{leastdeg-disc},
where it came from Formula~\eqref{BJ-G}
as $\Disc(\bar G)$,
and once from the definition
of $\redDisc(H)$,
which explains the square
in Formula~\eqref{eq:generalizedSalmonFormula}.
In the discussion following Definition~\ref{defn:reddisc} above,
we explained that, in that definition,
$\Disc(F_s)$ is a geometrically meaningful term,
as $F_s$ is the equation of the tangent cone of $\V(H)$ at the origin,
whereas $\Disc(F_d)$ is a technical artefact.
It is thus fortunate that
the latter term does not appear in
Formula~\eqref{eq:generalizedSalmonFormula}. Note that, indeed, the
factor $\Disc(F_d)$ in the definition of $\redDisc(H)$ cancels out
with the same factor coming from Formula~\eqref{BJ-F} as
$\Disc(\bar F)$.


\bigskip
Corollary~\ref{cor:generalizedSalmonFormula}
provides an interesting connection between ordinary
and reduced discriminants. As a first illustration of its interest, we
give the following generalized weight properties of the reduced
discriminant, which generalize the computations of
Example~\ref{ex:reddiscn=1} to arbitrary $n$.


\begin{proposition}
\label{pr:weight-reddisc}
\phantom{.}
\subparagraph{}
\label{pr:weight-reddisc.a}
In the grading of $\AZ$ defined by $\weight(U_\balpha)=\alpha_0$, 
the reduced discriminant $\redDisc_d^s (F)$ is homogeneous of degree
\[
  d(d-1)^n-(s-1)^{n-1}
  \bigl[ d\,\bigl((n+1)s+n-1\bigr)
  -ns(s+1)
  \bigr].
\]
\subparagraph{}
\label{pr:weight-reddisc.b}
In the grading of $\AZ$ defined by $\weight(U_\balpha)=d-\alpha_0$, 
the reduced discriminant $\redDisc_d^s (F)$ is homogeneous of degree
\[
n\bigl[
d(d-1)^n - s(s+1)(s-1)^{n-1}
\bigr].
\]
\end{proposition}


\begin{proof}
In the two gradings of \ref{pr:weight-reddisc.a} and
\ref{pr:weight-reddisc.b}, the plain discriminant $\Disc(F)$ is
homogeneous. Thus all its summands are homogeneous, and in particular
its piece of lowest degree in the Zariski grading is
homogeneous. We shall see that $\Disc(G)$ and $\Disc(F_s)$ are
homogeneous as well. Therefore,
it follows from Formula~\eqref{eq:generalizedSalmonFormula} that
$\redDisc(H)$ is homogeneous. Then it is only a matter of computing
its degree.

In the grading of \ref{pr:weight-reddisc.a}, 
$\Disc_d(F)$ has weight $d(d-1)^n$ by
Proposition~\ref{par:weightdisc}.
One has
\(
G = X_0^{s}F_0+X_0^{s-1}F_1+\cdots+F_s
\)
and the coefficients of $F_i$ have weight $d-i
=(s-i)+(d-s)$,
hence $\Disc_d(G)$ has weight 
\[
  s(s-1)^n+(n+1)(d-s)(s-1)^n
\]
by Proposition~\ref{par:weightdisc} and Corollary~\ref{c:further-wt-disc}.
The coefficients of $F_s$ all have weight $d-s$, 
hence $\Disc_s(F_s)$ has weight
\[
  n(d-s)(s-1)^{n-1}
\]
by the homogeneity property of the discriminant in Definition~\ref{def:disc}
and Corollary~\ref{c:further-wt-disc}
(note that $\Disc_s(F_s)$ is a discriminant for polynomials in $n$
indeterminates, \ie one less than $\Disc_d(F)$ and $\Disc_d(G)$).
One thus finds, by the above
Corollary~\ref{cor:generalizedSalmonFormula},
that $\redDisc_d^s (F)$ is homogeneous of degree
\begin{multline*}
  d(d-1)^n
  - s(s-1)^n-(n+1)(d-s)(s-1)^n
  - 2n(d-s)(s-1)^{n-1}
  \\
  \begin{aligned}
    &=
    d(d-1)^n-(s-1)^{n-1}
    \bigl[ s(s-1)+(n+1)(d-s)(s-1)
    +2n(d-s)
    \bigr]
    \\
    &=
    d(d-1)^n-(s-1)^{n-1}
    \bigl[ d\,\bigl((n+1)s+(n-1)\bigr)
    -ns(s+1)
    \bigr].
  \end{aligned}      
\end{multline*}

In the grading of \ref{pr:weight-reddisc.b},
$\Disc(F)$ is homogeneous
of degree $nd(d-1)^n$ by Proposition~\ref{par:weightdisc},
and $\Disc(G)$ is homogeneous of degree
$ns(s-1)^n$ by the same result. 
In addition, all the coefficients of $F_s$ have weight
$s$ in this grading hence, by the homogeneity property given in
Definition~\ref{def:disc}, 
$\Disc(F_s)$ is homogeneous of degree $ns(s-1)^{n-1}$
(note that $F$ is a homogeneous polynomial in $n$ variables only).
Then the conclusion follows by a direct computation.
\end{proof}

% pour vérifier les calculs :
% s*(s-1)+(n+1)*(d-s)*(s-1)+2*n*(d-s)
% d*((n+1)*s+(n-1))-n*s*(s+1)

For $n=1$, the degree in \ref{pr:weight-reddisc.a} is
\[
  d(d-1)-
  \bigl[ 2sd  -s(s+1)
  \bigr]
  = d^2-(2s+1)d+s(s+1),
\]
which agrees with \eqref{reddisc-n1-a},
and the degree in \ref{pr:weight-reddisc.b}
agrees with \eqref{eq:redDiscn=1}.


\bigskip
% \paragraph{Comment}
% \label{com:future}
In the above paragraphs we have introduced the reduced discriminant
and provided some first properties that are sufficient for our
purposes. A more detailed and complete study of this new
eliminant polynomial, including for instance its irreducibility and
the geometric meaning of its vanishing, in particular its connection
to Milnor number, will appear in \cite{BD2}.

% seems worthwhile and is left for future
% work.\footnote
% {In fact, so many years have passed since the first writing of this
%   text, that this has now been carried out, see \cite{BD2}.}


\subsection{Application to the Salmon Formula}
\label{s:app-to-Salmon}

We shall now see that Salmon's formula 
\taylordisc{} %\eqref{taylor-discr}
is a particular case of the decomposition formula given in Corollary
\ref{cor:generalizedSalmonFormula}.
We will then be able to generalize it to
the case of a hypersurface in arbitrary dimension.


\paragraph{Original Salmon Formula}
Let $F(X,Y,Z)$ be the generic homogeneous polynomial of degree $d\geq
3$, and set
\begin{gather*}
F=X^d F_0+X^{d-1}F_1+X^{d-2}F_2+\cdots+ X F_{d-1}+F_d, \\
F_0=U, \qquad F_1(Y,Z)=SY+TZ, \qquad
F_2(Y,Z)=\frac{1}{2}(A{Y}^{2}+2BYZ+C{Z}^{2});
\end{gather*}
(we introduce a rational number in the definition of $F_2$ to
follow Salmon's notation; this is natural in terms of the
Taylor--Newton Formula of
\cite[Paragraph~\tref{p:Taylor-Newton}]{13.th-classic}). 

We consider the truncation of $F$ at order $d-2$ with respect to $X$,
and the corresponding Zariski grading. So, $U$ has degree 2, $S$ and
$T$ have degree 1, and the coefficients of the $F_k$'s with $k\geq 2$
have degree $0$ (this includes the coefficients $A,B,C$). We let
\[
H= X^{d-2}F_2+\cdots+XF_{d-1}+F_d
\quad \text{and} \quad
G=X^2F_0+XF_1+F_2.
\]
Then, Corollary \ref{cor:generalizedSalmonFormula} tells us that 
\begin{equation}
\label{gnlzd-salmon-trunc2}
\Disc(F)= \Disc(G)\, \Disc(F_2)^2\, \redDisc(H) +
\bigl(\text{terms of Zariski weight}\geq 3 \bigr).
\end{equation}
Discriminants of quadratic forms are readily computed, see, \eg
\cite[\no 5 Exemple~6, p.~363]{demazure}, which is based on
Identity \eqref{def:disc:eq};
one has
\[
\Disc(F_2)=
\begin{vmatrix}
A & B \\ B & C
\end{vmatrix}
= AC-B^2,
\]
and
\[
\Disc(G)
=
\frac 1 2 \cdot
\begin{vmatrix}
2U & S & T \\
S & A & B \\
T & B & C 
\end{vmatrix}
= \frac{1}{2} \left( 2ACU- A{T}^{2}
  -2{B}^{2}{U} +2 BST- C{S}^{2} \right).
\]
Thus, Display~\eqref{gnlzd-salmon-trunc2} reads
\begin{multline*}
\Disc(F)= 
\frac{1}{2}
 \left( 2ACU- A{T}^{2}
  -2{B}^{2}{U} +2 BST- C{S}^{2} \right)
\cdot \left(AC-B^2\right)^2
\cdot \redDisc(H) \\
\mod \bigl( (S,T)^3+U(S,T)+(U^2) \bigr).
\end{multline*}
% M = matrix({{2*u,s,t}, {s,a,b},{t,b,c}})
% det M
Then, the specialization $U=S=0$ yields
\begin{equation}
\label{taylordiscr-corr}
\Disc(F)= 
-\frac{1}{2}
A\,{T}^{2}
\cdot \bigl(AC-B^2\bigr)^2
\cdot \redDisc(H) 
\quad \mod (T^3);
\end{equation}
this is Salmon's Formula 
\taylordisc{}, with the normalization factor $-\frac 1{2}$,
and with $\Phi = \redDisc(H)$.
% We mention that computations in the cases $d=2$ and $d=3$ with a
% computer algebra system have shown that $\redDisc(H)$ is an
% irreducible polynomial in these two cases.

\paragraph{Salmon Formula in arbitrary dimension} 
\label{p:taylor-discr-arbdim}
The Salmon Formula for the discriminant of a plane curve can be
generalized to the case of a hypersurface in a projective space of
arbitrary dimension as follows.
In a suitable system of homogeneous coordinates, any hypersurface
$\V(F)\subset \P^n$ has an equation of the form
\begin{equation}
\label{eq:hypsf-nmform}
F(X_0,X_1,\ldots,X_n)
=T X_0^{d-1}X_n+\sum_{k=2}^d X_0^{d-k}F_k(X_1,\ldots,X_n),
\end{equation}
where for all $k=2,\ldots,d$, the polynomial $F_k$ is homogeneous
of degree $k$ in the indeterminates $X_1,\ldots,X_n$.
This normal form merely imposes that the hypersurface $\V(F)$
goes through the point $(1:0:\cdots:0)$ and that its tangent
hyperplane at this point is given by $X_n=0$. Applying 
Corollary~\ref{cor:generalizedSalmonFormula} as above, and setting
$H=\sum_{k=2}^d X_0^{d-k}F_k$, we find that
$$ \Disc(F)=\Disc(TX_0X_n+F_2)\, \Disc(F_2)^2\, \redDisc(H) \quad \mod T^3.$$ 

Let $\bar F_2(X_1,\ldots,X_{n-1})$ be the homogeneous polynomial
of degree $2$ in the indeterminates $X_1,\ldots,X_{n-1}$ defined as 
\[
  \bar F_2(X_1,\ldots,X_{n-1}) =F_2(X_1,\ldots,X_{n-1},0)
\]
(beware the difference in notation with \ref{p:ident-disc}).
We have:
\begin{align}
  \hspace{5mm}
  \rlap{$2^{a(n,2)}\,\Disc(TX_0X_n+F_2)$}
  \hspace{15mm}
  \notag \\
  & =
\Res\bigl( \partial_0(TX_0X_n+F_2),\, \partial_1(TX_0X_n+F_2),\, 
    \ldots,\, \partial_n(T X_0 X_n+F_2) \bigr)
  \notag \\
& =
\Res\bigl( TX_n,\, \partial_1 F_2,\, 
\ldots,\, \d{n-1} F_2,\,
T X_0 +\d{n}F_2 \bigr)
  \notag \\
& = -\Res\bigl( T X_0 +\d{n}F_2,\, \partial_1 F_2,\, 
\ldots,\, \d{n-1} F_2,\,
              TX_n \bigr)
  \label{salmon:exchange} \\
  & = -T \cdot \Res\bigl( TX_0+ \restr {\partial_n F_2} {X_n=0},\,
    \restr {\partial_1 F_2} {X_n=0},\,  
\ldots,\,  \restr {\partial_{n-1} F_2} {X_n=0}
    \bigr)
  \label{salmon:section} \\
& = -T^2 \cdot \Res(\partial_1 \bar F_2,\, \ldots,\,  
\partial_{n-1} \bar F_2) 
= -2^{a(n-2,2)} \, T^2 \cdot \Disc(\bar F_2),
\label{salmon:laplace}
\end{align}
where:
\begin{compactitem}[---]
\item the exponents $a(n,2)$ and $a(n-2,2)$ are as defined in
  \ref{def:disc}; 
\item \eqref{salmon:exchange} is obtained by
  \cite[\S 5.8, Effet d'une permutation des polynômes]{J91};
\item \eqref{salmon:section} is obtained by \cite[(5.13.5)]{J91};
\item \eqref{salmon:laplace} is obtained by \cite[\S 5.10, Formule de
  Laplace]{J91}.
\end{compactitem}
Alternatively, since the resultants above are resultants of
homogeneous polynomials of degree $1$ they may be computed as
determinants, see \cite[\S 5.3, Cas des formes linéaires]{J91}, to the
effect that
\begin{equation}
\label{salmon:discriminant}
\Res\bigl( TX_n,\, \partial_1 F_2,\, 
\ldots,\, \d{n-1} F_2,\,
T X_0 +\d{n}F_2 \bigr)
=
\begin{vmatrix}
  0 & 0 & \cdots & \cdots & 0 & T \\
  0 & \lbrack\phantom{A} & & \d{1}F_2 &  & \phantom{A}\rbrack \\
  \vdots & & &\vdots &  \\
  0 & \lbrack\phantom{A} & & \d{n-1}F_2 &  & \phantom{A}\rbrack
  \\
  T & \lbrack\phantom{A} & & \d{n}F_2 &  & \phantom{A}\rbrack
\end{vmatrix},
\end{equation}
where each ``$\lbrack\ \d{i}F_2\ \rbrack$'' denotes the line
containing the $n$ coefficients of $\d{i}F_2$ in the indeterminates
$X_1,\ldots,X_n$;
from formula \eqref{salmon:discriminant} one may easily retrace the
previous computations.

Either way, the upshot is that
$\Disc(TX_0X_n+F_2)=-T^2\,\Disc(\bar F_2)$
(note that $a(n,2)=a(n-2,2)$), and 
eventually we obtain the following generalized Salmon formula:
\begin{equation}\label{eq:Salmonhypersurface}
  \Disc(F)=-T^2\,\Disc(\bar F_2)\,\Disc(F_2)^2 \redDisc(H)
  \quad\mod T^3.
  %+ T^3 \psi.
\end{equation}
In the situation of the original Salmon Formula
above, one has
$F_2(Y,Z) = \frac 1 2(AY^2+2BYZ+CZ^2)$ and
$\bar F_2(Y) = \frac 1 2 AY^2$,
hence $\Disc(F_2) = AC-B^2$ and
$\Disc(\bar F_2) = \frac 1 2 A$,
and thus the two formulas \eqref{taylordiscr-corr}
and \eqref{eq:Salmonhypersurface}
are coherent.


\section{Computation of the node-couple degree by 
elimination}
\label{S:salmon's-comput}

In \cite[\S605--607]{salmon2_16}, Salmon sets up the following strategy
to compute the number of $2$-nodal curves in a general net of
hyperplane sections of a smooth (hyper)surface $S \subset \P^3$.
For $p' \in S$ and $p'' \in \T_{p'}S -\{p'\}$, consider the pencil 
$\orth {\vect {p',p''}} \subset \check \P^3$ of (hyper)planes
containing $p'$ and $p''$.
It cuts out $\dual d=\deg (\dual S)$ points on the dual
surface $\dual S$,
counted with multiplicities, which correspond to planes tangent to
$S$. 
Among these, $\T _{p'} S$ counts doubly if it is a plain tangent
plane, and triply if it is plainly bitangent. 

Indeed, the line $\orth {\vect {p',p''}}$ is contained in the plane
$\orth {(p')}$, hence tangent to $\dual S$ at the point 
$\orth {(\T_{p'}S)} \in \dual S$.
If the plane $\T_{p'}S$ is plainly bitangent to $S$, then $\orth
{(\T_{p'}S)}$ is a general point on the ordinary double curve of
$\dual S$, and the line $\orth {\vect {p',p''}}$
is tangent to one of the two
transverse sheets of $\dual S$ at $\orth {(\T_{p'}S)}$.
The idea is then to determine first the conditions on $p'$ for 
$\T _{p'} S$ to count with multiplicity greater than $2$ in 
$\orth {\vect {p',p''}}$, and then to sort out the various
corresponding geometric situations. A key element to carry this out is
the famous formula \taylordisc{}; another one is the
elimination procedure \ref{p:elim-lambdamumu}.

We work out Salmon's procedure in subsection~\ref{s:salmon-thecomput},
and in subsection~\ref{s:salmon-thecomput-arb} we show how it carries
over for hypersurfaces in a projective space of arbitrary dimension.
From now on, we work over an algebraically closed field $\k$ of
characteristic $0$.
We use freely the theory of polarity, on which there is a recap in the
previous chapter \cite[Appendix A]{13.th-classic}.

%\label{s:polarity}


\subsection{An elimination trick}
\label{s:salmon-trick}

This section is dedicated to an elimination trick due to Salmon,
see \cite[\S 606]{salmon2_16}.
It is the main technical device that he uses to conduct his study of
pencils of planes orthogonal to a tangent line, which eventually gives
the node-couple degree. We advise the reader to skip this section in
first reading and move on to Section~\ref{s:salmon-thecomput} where
the general picture of Salmon's approach is given, and to come back
here only when needed.
% Our treatment here is a vast expansion of Salmon's arguments, as he
% leaves aside some important verifications, probably following the
% standards of his time.


\paragraph{}
\label{p:setup-salmon's-trick}
Let $\k$ be an algebraically closed field of characteristic 
$0$, and
consider a smooth, degree $d$, surface $S \subset \P^3$
defined by a homogeneous polynomial $F\in \k[X,Y,Z,W]$;
set
\[
\Tan S
=\bigl\{ (p',p''):
p'\in S
\text{ and }
p'' \in \T_{p'}S
\bigr\}
\, \subset \, \P^3\times \P^3.
\]

Let $\Phi_{\hat p', \hat p''}(\hat p)$ be a trihomogeneous polynomial
in the sets of variables 
$(\hat p', \hat p'', \hat p) \in (\k^4)^3$,
of tridegree $(\lambda, \mu, \mu)$
for some non-negative integers $\lambda, \mu$.
Assume that for all 
$(p',p'') \in \Tan S$, $p'\neq p''$,
the hypersurface $\V(\Phi_{\hat p',\hat p''}) \subset \P^3$ consists of
$\mu$ planes, counted with multiplicities, all containing the line 
$\vect {p',p''}$.

\begin{theorem}
\label{p:elim-lambdamumu}
Let $p'$ be a point of $S$. The following assertions are equivalent:
\begin{compactenum}[(i)]
\item there exists $p'' \in \T_{p'}S - \{p'\}$ such that the tangent plane 
$\T_{p'}S$ is a component of $\V(\Phi_{\hat p',\hat p''})$;
\item
for all $p'' \in \T_{p'}S - \{p'\}$,
$\T_{p'}S$ is a component of $\V(\Phi_{\hat p',\hat p''})$.
\end{compactenum}
Moreover, there exists a homogeneous polynomial $G\in \k[X,Y,Z,W]$
of degree $\lambda+(d-2)\mu$ such that (i) and (ii)
are equivalent to:
\begin{compactenum}[(i)]
\setcounter{enumi}{2}
\item
$p'$ lies on the hypersurface $\V(G) \subset \P^3$.
\end{compactenum}
\end{theorem}

We need some preparation for the proof.
We begin with the following characterization of the non-emptiness of
the intersection of two lines in $\P^3$, one given parametrically and
the other defined by equations.

\begin{lemma}\label{lem:linesIntersection}
Let $L', L'' \in \k[X,Y,Z,W]$ be two linear functionals,
and $\hat p', \hat p'' \in \k^4$.
The intersection of the two lines $\V(L',L'')$ and 
$\vect {p',p''}$ is non-empty if
and only if 
\[
  D_{L',L''}(p',p'')
  \overset{\text{def.}}= 
  \begin{vmatrix}
  %\left|\begin{array}{cc}
  L'(\hat p') & L''(\hat p') \\
  L'(\hat p'') & L''(\hat p'')
  \end{vmatrix}
  %\end{array}\right|
  % =
  % \trsp {\hat a'} (\hat p')\cdot \trsp {\hat a''} (\hat p'') - \trsp
  % {\hat a'} (\hat p'') \cdot \trsp {\hat a''} (\hat p')
\]
vanishes. 
\end{lemma}

\begin{proof}
The line $\vect {p',p''}$ is the image of the map
$\P^1\rightarrow \P^3$ defined by the linear map
$(u,v)\in \k^2 \mapsto
u\hat p'+v\hat p'' \in \k^4$.
Therefore, the lines $\V(L',L'')$ and
$\vect {p',p''}$ intersect if and only if the two polynomials
$L'(u\hat p'+v\hat p'')$ and $L''(u\hat p'+v\hat p'')$
share a common root in $\P^1$. These polynomials are linear
forms in $u,v$, and the polynomial $D_{L',L''}(p',p'')$ is the
determinant of the corresponding linear system.
\end{proof}	

For all $L',L''$, $D_{L',L''}$ is a bihomogeneous polynomial in the
two sets of variables $(p',p'')$, of bidegree $(1,1)$ and
anti-symmetric; this implies that it is irreducible.

\begin{lemma}
\label{sueurs-froides}
For general linear forms $L',L''$, the intersection in
$\P^3\times \P^3$ of $\Tan S$ and the hypersurface $\V(D_{L',L''})$ is
integral.
\end{lemma}

\begin{proof}
A natural idea is to try and prove the lemma as an application of
Bertini's theorem. It is however delicate to proceed this way, as for
instance the map defined on $\P^3\times\P^3$ by the linear system of
anti-symmetric forms of bidegree $(1,1)$ is certainly not generically
finite, and even less so the map defined by the system of
all $D_{L',L''}$. We will thus rather prove the result by hand.

Let us first note that as $L',L''$ range through all linear forms,
the bihomogeneous forms $D_{L',L''}$ cover all rank $2$, bilinear,
anti-symmetric forms. This is a direct calculation: for
\[
  L' = A'X+B'Y+C'Z+D'W
  \et
  L'' = A''X+B''Y+C''Z+D''W,
\]
$D_{L',L''}$ is the bilinear form
\[
  \left(
  \begin{pmatrix}
    X'\\Y'\\Z'\\W'
  \end{pmatrix},
  \begin{pmatrix}
    X''\\Y''\\Z''\\W''
  \end{pmatrix}
  \right)
  \longmapsto
  (X',Y',Z',W')
  \begin{pmatrix}
    0 & U_{01} & U_{02} & U_{03} \\
    -U_{01} & 0 & U_{12} & U_{13} \\
    -U_{02} & -U_{12} & 0 & U_{23} \\
    -U_{03} & -U_{13} & -U_{23} & 0
  \end{pmatrix}
  \begin{pmatrix}
    X''\\Y''\\Z''\\W''
  \end{pmatrix}
\]
where the coefficients $U_{ij}$ are the six $2\times 2$ minors of the
matrix
\[
  \begin{pmatrix}
    A'&B'&C'&D' \\
    A''&B''&C''&D''
  \end{pmatrix}.
\]
It follows that the only relation between the coefficients $U_{ij}$
is the vanishing of the Pfaffian of the
anti-symmetric matrix $(U_{ij})$, \ie
\[
  U_{01}U_{23}
  -U_{02}U_{13}
  +U_{03}U_{12}
  =0
\]
(this is the Plücker equation of the Grassmannian $\Gr(2,4)$ in
$\P^5$).

Now to the lemma. Projection on the first factor in $\P^3\times\P^3$
makes $\Tan S$ a $\P^2$ bundle over $S$: for all $p'\in S$, the fibre
over $p'$ is the zero locus of the linear form $\dD_{p'}F$ (the
differential of $F$, a defining equation for $S$, at the point $p'$;
it is non-zero as we assume that $S$ is smooth).
Similarly, for all $p' \in \P^3$ the fibre
$\pr_1^{-1}(p')\cap \V(D_{L',L''})$ is the zero locus of the linear
form $D_{L',L''}(p', \,\_\,)$, which is either a hyperplane or the
whole $\P^3$.
We claim that for general $L',L''$, the intersection
$\Tan S \cap \V(D_{L',L''})$ is the closure of a $\P^1$-bundle over an
open subset of $S$, which implies at once that it is irreducible.
Moreover, this implies that the intersection
$\Tan S \cap \V(D_{L',L''})$
is fibrewise over $S$
a transverse intersection of hyperplanes, and therefore it is reduced.
Thus the claim proves the lemma.
To prove the claim it suffices to show that,
for general $L',L''$, the set of points
$p'\in S$ such that the linear form $D_{L',L''}(p', \,\_\,)$ is a
multiple of $\dD_{p'}F$ has dimension $0$; in particular, the
intersection $\Tan S \cap \V(D_{L',L''})$ cannot have any irreducible
component generically a $\P^2$-bundle over a curve in $S$.

The claim follows from explicit computations. The two linear forms
$\dD_{p'}(F)$ and $D_{L',L''}(p', \,\_\,)$ are, in coordinates,
\[
  \bigl( \partial_XF(p'), \, \partial_YF(p'),
  \,\partial_ZF(p'), \,\partial_WF(p')
  \bigr)
  \et
  \begin{pmatrix}
    X''\\Y''\\Z''\\W''
  \end{pmatrix}
  ^{\kern -.3em \mathsf T}
  \cdot
  \begin{pmatrix}
    0 & U_{01} & U_{02} & U_{03} \\
    -U_{01} & 0 & U_{12} & U_{13} \\
    -U_{02} & -U_{12} & 0 & U_{23} \\
    -U_{03} & -U_{13} & -U_{23} & 0
  \end{pmatrix}.
\]
Both have the line $p' \subset \k^4$ in their kernel, so we consider
the corresponding linear forms on the quotient $\k^4\big/ p'$, given
by line matrices with three entries; up to a linear change of
coordinates we may assume that $p'=(0:0:0:1)$, in which case we are
simply forgetting the last entry in the two above line matrices.
The claim then boils down to the fact that the three $2\times 2$
minors of the $2\times 3$ matrix obtained by concatenating the two line
matrices corresponding to $\dD_{p'}(F)$ and $D_{L',L''}(p', \,\_\,)$
define a locus of codimension at least two on $S$, for general
$L',L''$.
Since everything is explicit, one may observe that for a general
choice of $L',L''$, any two of these three minors have no common
factor, which proves the claim.
% We believe it is best to let the reader write down this 
% elementary verification on her or his own.
\end{proof}




% \begin{proof}[Proof of Theorem~\ref{p:elim-lambdamumu}]
\paragraph{Proof of Theorem~\ref{p:elim-lambdamumu}}
The proof is based on the
fact that 
$\T_{p'}S$ is a component of $\V(\Phi_{p', p''})$
if and only if, for all line $\Lambda \subset \P^3$ 
the intersection $L \cap \T_{p'}S \cap \V(\Phi_{p', p''})$
is non-empty; a moment of thought should convince the reader that this
fact is indeed true.
Then the idea is to consider a suitable resultant to express this
fact, and to factor a power of $D_{L',L''}(p',p'')$ out of this
resultant. 

Consider $T_{p'}= \polar { p}F ( p')$ as a trihomogeneous
polynomial of tridegree $(d-1,0,1)$ in $( p', p'', p)$.
Let $L', L'' \in \check\P^3$ be two generic linear forms in $p$,
and consider the line
$\Lambda = \V(L',L'')$ in $\P^3$.
It intersects $\T_{p'}S \cap \V(\Phi_{ p', p''})$ if and only if
the resultant 
\[
  R=\Res(T_{p'}, \Phi_{p',p''}, L', L''),
\]
with respect to the set of
variables $p$, vanishes.
It follows from
the homogeneity properties of the resultant, see Theorem~\ref{T:res},
that $R$ is a multi-homogeneous polynomial in the sets of variables 
$(L', L'',  p', p'')$, of multi-degree
$(\mu,\mu,\mu(d-1)+\lambda,\mu)$.
% (we identify $L'$ and $L''$ with
% the datum of their coefficients in $X,Y,Z,W$).

For a given $(p',p'') \in \Tan S$, the polynomial $\Phi_{p',p''}$
splits as the 
product of $\mu$ linear forms $\Phi^i_{p',p''}$, $i=1,\ldots,\mu$,
that all vanish along the line $\vect {p',p''}$.
Although this splitting may not exist globally over $\Tan S$
(in other words the factors $\Phi^i_{p',p''}$ may not be polynomials in 
$(p',p'')$),
there exists a global splitting over a finite cover
$\tilde {\Tan S}$ of $\Tan S$\footnote
{\def\cP{\mathcal{P}}
let us briefly recap how such a finite cover may be constructed. The
family of planes defined over $\Tan S$ by $\Phi_{p',p''}$
corresponds to a subscheme $\cP$ of $\Tan S \times \check{\P^3}$
with the first projection inducing a degree $\mu$ map $\cP \to \Tan
S$. Our goal is to show that there exists a base change
$\tilde{\Tan S} \to \Tan S$ such that
$\cP \times_{\Tan S} \tilde{\Tan S}$ splits as $\mu$ copies of
$\tilde{\Tan S}$. As a first step, we consider the following
(somewhat absurd non-sensical) base change.
\[
\xymatrix@=1em{
  \cP \times_{\Tan S} \cP \ar[r] \ar[d] & \cP \ar[d] \\
  \cP \ar[r] & \Tan S
}
\]
The diagonal $\Delta$ provides a section of the degree $\mu$ map
$\cP \times_{\Tan S} \cP \to \cP$,
hence $\cP \times_{\Tan S} \cP$ splits as $\Delta + \cP'$ where $\cP'$
comes with a degree $\mu-1$ map to $\cP$.
Then, by induction on $\mu$, one may construct a finite cover
$\tilde {\cP} \to \cP$ such that
$\cP' \times_{\cP} \tilde{\cP}$ splits as $\mu-1$ copies of
$\tilde{\cP}$, hence $\cP \times_{\Tan S} \tilde{\cP}$ splits as $\mu$
copies of $\tilde{\cP}$.
Thus $\tilde{\cP}$ is suitable as the $\tilde{\Tan S}$ we were
looking for. We point out the (non-accidental) similarity of this
construction with that of a splitting field for a given polynomial $P$
in one indeterminate $X$. The first base change in our construction is
the analogue of the field extension $\k[X]/(P)$. Also note that, in
general, the map $\tilde{\Tan S} \to \Tan S$ will have degree $\mu!$.} 
(in other words the factors $\Phi^i_{p',p''}$ have their coefficients
in a finite extension of $\k[p',p'']$).
Then, by the multiplicativity property,
see \cite[\S~5.7, p.~154]{J91},
the resultant $R$ splits as the product of the $\mu$ resultants
$R_i = \Res(T_{p'},\Phi^i_{p',p''}, L', L'')$.
By Lemma~\ref{lem:linesIntersection},
for all $i$ the resultant $R_i$ 
vanishes wherever $D_{L',L''}$ vanishes on $\Tan S$, or rather on
$\tilde {\Tan S}$, as both forms $T_{p'}$ and $\Phi^i_{p',p''}$ vanish
along the line $\vect {p',p''}$.
By Lemma~\ref{sueurs-froides}, this implies that $D_{L',L''}$
divides $R_i$ as a function of $(p',p'') \in \tilde{\Tan S}$.
Eventually, the upshot is that
$(D_{L',L''})^\mu$ divides $R$, and since both
$D_{L',L''}$ and $R$ are well-defined as
functions of $(p',p'') \in {\Tan S}$, so is the quotient.
Therefore,
there exists a multi-homogeneous polynomial $R'$
in the sets of variables
$(L',L'',p',p'')$
such that after restriction to
$\check \P^3 \times \check \P^3 \times \Tan S$
one has 
$R=(D_{L',L''})^\mu R'$.
Computing degrees, one finds that $R'$ has multi-degree
$(0,0,\mu(d-2)+\lambda,0)$ in 
$(L',L'',p',p'')$,
which proves the theorem.
% \end{proof}
\qed





\subsection{Study of a pencil of planes orthogonal
  to a tangent line}
\label{s:salmon-thecomput}
% avant : "the computation"


\paragraph{General setup}
\label{p:setup-salmon}
We recall that $\k$ is assumed to be an algebraically closed field of characteristic 
$0$.
We let $S \subset \P^3$ be a smooth surface of degree $d$,
defined by a homogeneous polynomial $F(X,Y,Z,W)$.
We consider generic $4$-tuples
$\hat p' = (X',Y',Z',W')$, $\hat p'' =
(X'',Y'',Z'',W'')$, $\hat p = (X,Y,Z,W)$, and call $p',p'',p$
the corresponding points in $\P^3$
(beware the unusual distribution of the prime decorations).
The choice of 
$\hat p', \hat p'', \hat p$ defines a
system of homogeneous coordinates $(\alpha:\beta:\gamma)$ on the plane
$\vect {p',p'',p}$
generated by $p'$, $p''$ and $p$. We consider 
\begin{equation}
\label{taylor}
\begin{aligned}
  f(\alpha, \beta, \gamma)
  &\overset{\text{def.}}{=}
  F(\alpha \hat p' + \beta \hat p'' + \gamma \hat p)
  \\
&= \alpha ^d \cdot F(\hat p')
+ \alpha^{d-1} \cdot \polar {\beta \hat p''+\gamma \hat p} F(\hat p')
+ \frac 1 2 \alpha^{d-2} \cdot 
\polar {(\beta \hat p''+\gamma \hat p)^2} F(\hat p')
\ \mod (\beta,\gamma)^3
\\
&=  \alpha ^d \cdot F(\hat p')
+ \alpha ^{d-1} \bigl( \beta \polar {\hat p''}F(\hat p')
+ \gamma \polar {\hat p}F (\hat p') \bigr)
\\
&\qquad + \frac {1}{2} \alpha ^{d-2}
\bigl( \beta^2 \polar {\hat p''^2} F(\hat p') 
+2\beta\gamma \polar {\hat p''\hat p}F (\hat p')
+ \gamma^2 \polar {\hat
  p^2}F (\hat p') \bigr)
\quad \mod (\beta,\gamma)^3.
\end{aligned}
\end{equation}
Considered as a homogeneous polynomial in the variables
$(\alpha,\beta,\gamma)$, this is the equation of the hyperplane section of
$S$ by $\vect {p',p'',p}$.


\paragraph{Degree of the dual surface}
\label{p:deg-dual}
As a warm-up, let us derive the degree of the dual surface $\dual S
\subset \smash{\check \P^3}$ of $S$ from the relevant homogeneity
property of the discriminant.
We specialize $p'',p$ to two general points of $\P^3_\k$.
Then the coefficients of $f(\alpha,\beta,\gamma)$ are polynomials in
the set of indeterminates $\hat p' = (X',Y',Z',W')$, and so is the
discriminant $\Disc(f)$ with respect to the variables $\alpha, \beta, \gamma$.
The latter vanishes at a point $p' \in \P^3_\k$ if and only if the
plane $\vect {p',p'',p}$ is tangent to $S$.
Thus the zero locus $\V\bigl(\Disc(f)\bigr) \subset \P^3_\k$ is the
union of all planes tangent to $S$ and containing the line
$\vect{p'',p}$; in particular the degree of $\Disc(f)$ (as a
polynomial in $p'$, what else?) is the number of tangent planes to $S$
containing the line $\vect{p'',p}$, which is the degree of the dual
surface $\dual S \subset \smash{\check \P^3}$. This is also the number
of points in the intersection of $\dual S$ with the line
$\orth[p'',p] \subset \smash{\check \P^3}$,
the latter parametrizing planes passing through $p''$ and $p$.

The coefficient of $f(\alpha,\beta,\gamma)$ in
$\alpha^a\beta^b\gamma^c$
is a polynomial of degree $a$ in the set of indeterminates $\hat p'$,
as can be seen on the Taylor--Newton expansion, the first terms of
which are given in Display~\eqref{taylor}.
Therefore, by \ref{par:weightdisc.a}, the discriminant
$\Disc(f)$ is homogeneous of degree $d(d-1)^2$ in $\hat p'$,
and the dual surface $\dual S$ has degree $\dual d = d(d-1)^2$ in
$\smash{\check \P^3}$.

\begin{remark}
\label{rk:tridegree-disc}
If we let all three points (or $4$-tuples) $p',p'',p$ be generic, then
$\Disc( f(\alpha,\beta,\gamma))$ is tri-homogeneous with
respect to the three sets of indeterminates $p',p'',p$, of tri-degree
\[
  (\dual d, \dual d, \dual d) =
  ( d(d-1)^2, d(d-1)^2, d(d-1)^2),
\]
as follows from the
above analysis. Note that obviously $p',p'',p$ play symmetric roles in
the definition of $f$.
\end{remark}


In order to enumerate bitangent planes, we will take points
$p',p''$ such that the line $\vect{p',p''}$ is tangent to $S$ at $p'$,
and consider a reduced discriminant of the corresponding
$f(\alpha, \beta, \gamma)$.
Thus we need to specialize our setup a little.


\paragraph{The ``tangent line'' setup}
In the situation set-up in Paragraph~\ref{p:setup-salmon}
above,
we specialize $p'$ to the general point of $S$,
and $p''$ to the general point of $\T_{p'}S$.
Then $F(\hat p') = \polar {\hat p''}F(\hat p') =0$, 
so \eqref{taylor} reduces to
\begin{equation}
\label{taylor-red}
f(\alpha, \beta, \gamma) =
%f(\alpha \hat p' + \beta \hat p'' + \gamma \hat p) =
T \alpha ^{d-1} \gamma +
\frac {1}{2} \alpha ^{d-2} (A \beta^2 + 2B \beta\gamma + C \gamma ^2)
\quad \mod (\beta,\gamma)^3,
\end{equation}
where
$T= \obspolar {\hat p}f (\hat p')$,
$A= \obspolar {\hat p''^2} f(\hat p')$,
$B= \obspolar {\hat p''\hat p}f (\hat p')$,
$C= \obspolar {\hat p^2}f (\hat p')$.
Note in particular that, as homogeneous polynomials in the
set of indeterminates $\hat p=(X,Y,Z,W)$, $T$ and $C$ are the equations of
the tangent plane $\T_{p'} S$, and the polar quadric $\Polar^2S(p')$ 
of $S$ at $p'$, respectively.

We consider the discriminant of the plane curve
$S \cap \vect {p',p'',p}$, \ie the discriminant of
$f \in A[\alpha,\beta,\gamma]$ with $A=\k[X,Y,Z,W]$; by Formula \taylordisc{},
or rather Formula~\eqref{taylordiscr-corr}, it writes
\begin{equation}
\label{discr}
\Disc (f)
% \bigl( f(\alpha \hat p' + \beta \hat p'' + \gamma \hat p)
% \bigr)
= -\frac 1 {2}\, T^2 \bigl( A(B^2-AC)^2\,\Phi+T\,\Psi \bigr),
\et[\text{with}]
\Phi = \redDisc_d^{2}(f).
\end{equation}
As explained in the previous paragraphs, 
it vanishes if and only if the plane $\vect {p',p'',p}$ is tangent to
$S$; It is a trihomogeneous polynomial in the variables $\hat p'$,
$\hat p''$ and $\hat p$; as a polynomial in $p$,
it vanishes along the $\dual d$ planes (counted with multiplicities)
tangent to $S$ in the pencil
$\orth[p',p''] \subset \smash{\check \P^3}$ of planes containing the 
line $\vect{p',p''} \subset \P^3$.


\begin{remark}
\label{rk:bidual-tg-line}
The fact that $T^2$ factors out of $\Disc(f)$
gives an algebraic proof of the fact that the tangent plane
$\T_{p'}S$ appears with multiplicity $\geq 2$ in the scheme
$\orth[p',p''] \cap \dual S$; or rather, the point
$\orth[\T_{p'}S] \in \smash{\check \P^3}$
appears with multiplicity $\geq 2$ in the scheme
$\orth[p',p''] \cap \dual S$.

In other words, if a line $\Lambda \subset \P^3$ is tangent to $S$ at
some point $p$, then the line
$\orth \Lambda \subset \smash{\check \P^3}$ is tangent to the dual
surface $\dual S$ at the point $\orth[\T_{p}S]$.
\end{remark}


Salmon's idea is that if the tangent plane
$\T_{p'}S$ is also tangent to $S$ at some point different from $p'$,
then it should appear with multiplicity $>2$ in
$\orth[p',p''] \cap \dual S$;
equivalently, $\Disc(f)$ should be divisible by $T^3$ in the above
setup. 

Therefore, we shall now discuss the various possibilities for $T$ to
divide 
$A(B^2-AC)^2\,\Phi$, in the notation of Equation~\eqref{discr}.



\paragraph{Vanishing of $A$ and biduality for inflectional tangents}
\label{p:vanishing-2nd-polar}
The polynomial $A$ has degree $0$ in $p$, therefore it is divisible by
$T$ if and only if it is identically zero.
By definition $A= \polar {\hat p''^2} f(\hat p')$, so its vanishing is
equivalent to the point $p''$ being on the polar quadric 
$\Polar_{{p'}^2} S$ of $S$ at $p'$. Since $p'' \in \T_{p'}S$, this in turn is equivalent
to the line $\vect{p',p''}$ being one of the two inflectional tangents
of $S$ at $p'$
(\ie
the two lines $\Lambda$ having intersection multiplicity with $S$ at
$p'$ at least $3$; in symbols,
$i( \vect{p',p''},S)_{p'} \geq 3$).

We thus find an algebraic proof of the fact that
\[
  \text{if}\quad
  i\bigl( \vect{p',p''},S \bigr)_{p'} \geq 3,\quad
  \text{then}\quad
  i\bigl( \orth[p',p''], \dual S \bigr)_{\orth{(\T_{p'}S)}} \geq 3,
\]
which is a manifestation of biduality.
Geometrically, if a line $\Lambda \subset \P^3$ is an inflectional
tangent to $S$ at $p'$ (\ie $L$ is the tangent line to one of the two
local branches of $\T_pS \cap S$ at $p'$),
then its orthogonal $\orth \Lambda \subset \check \P^3$
is an inflectional tangent to $\dual S$ at the point
$\orth {(\T_{p'}S)}$. 

As a side remark note that when $A=0$, all the curves cut out on $S$ by
a member of the pencil $\orth[p',p'']$ have an inflection point at $p'$.

\paragraph{} 
\label{p:lambdamumu-aux}
We shall analyze the divisibilities of $B^2-AC$ and $\Phi$ by $T$
using Theorem~\ref{p:elim-lambdamumu}.
To see that the latter result indeed applies, we note that 
for $(p',p'') \in \Tan S$ (see the notation in
Paragraph~\ref{p:setup-salmon's-trick}),
the discriminant in Display~\eqref{discr},
$T^2A(B^2-AC)^2\Phi+T^3\Psi$, 
defines as a homogeneous polynomial in
the variable $p$ a hypersurface consisting of $\dual d$
planes, counted with multiplicities, all containing the line
$\vect {p',p''}$. 
This implies
that so does its homogeneous piece of lowest degree with respect to
any grading, as the piece of lowest degree of a product is the product
of the pieces of lowest degree.
For the Zariski grading, see subsection~\ref{s:app-to-Salmon},
the piece of lowest degree of the discriminant is
$T^2A(B^2-AC)^2\Phi$.
The upshot is that $T^2A(B^2-AC)^2\Phi$, as a polynomial in $p$,
defines a sum of planes, all containing the line $\vect {p',p''}$,
which implies that so do all the factors $T,A,B^2-AC,\Phi$.

Note that this is obvious for $T$, which defines the plane $\T_{p'}S$.
The polynomial $A$, on the other hand, is
independent on the variable $p$, hence defines either the whole
space, or the empty set.

\paragraph{Divisibility of $B^2-AC$ by $T$ and biduality at parabolic
  points} 
\label{p:divB^2-AC}
The polynomial $B^2-AC$ is tri-homogeneous of tri-degree 
$(2(d-2),2,2)$ in the variables $(p',p'',p)$.
By Theorem~\ref{p:elim-lambdamumu}, arguing as in 
Paragraph~\ref{p:lambdamumu-aux} above,
there exists a homogeneous polynomial $H$ of degree $4(d-2)$ in
the variable $p'$, with constant coefficients, such that
for fixed $p' \in S$ and $p'' \in \T_{p'}S$, $T$ divides $B^2-AC$ as
polynomials in $p$ if and only if $H(p')=0$.

The polynomial $H$ is, in fact, the Hessian determinant.
Indeed, it follows from 
\eqref{taylor-red} that the tangent cone of the section of $S$ by its
tangent hyperplane at $p'$,
$S \cap \T_{p'}S$,
is defined by the quadratic form given by the symmetric matrix
\[
\begin{pmatrix}
A & B \\ B & C
\end{pmatrix}.
\]
Thus, $B^2-AC$ is zero modulo $T$ if and only if the curve 
$S \cap \T_{p'}S$ has a degenerate tangent cone at $p'$,
\ie $p'$ is a parabolic point of $S$.

Geometrically this is explained as follows. If $p'$ is a parabolic
point of $S$, then the point $\orth{(\T_{p'}S)}\in \check \P^3$ sits
on the cuspidal double curve of $\dual S$,
and for $p'' \in \T_{p'}S-\{p'\}$,
the line $\orth[p',p''] \subset \check \P^3$
is contained in the tangent cone of
$\dual S$ at the point $\orth{(\T_{p'}S)}\in \check \P^3$,
hence 
$i(\orth[p',p''], \dual S) _{\orth{(\T_{p'}S)}} \geq 3$.


\paragraph{Divisibility of the reduced discriminant $\Phi$ by $T$}
\label{p:div-redDisc}
The discriminant in Display~\eqref{discr}
is tri-homogeneous in the variables $(p',p'',p)$
with respect to the standard grading,
of degree $\dual d = d(d-1)^2$ 
with respect to all three variables, as we have observed above.
This implies that also the homogeneous piece of \eqref{discr}
of lowest degree with respect to the Zariski grading
is tri-homogeneous of tri-degree $(\dual d, \dual d, \dual d)$ for
the standard grading.
Moreover, $T$, $A$, and $B^2-AC$ have respective tri-degrees
$(d-1,0,1)$, $(d-2,2,0)$, and $(2(d-2),2,2)$
in $(p',p'',p)$.
Thus, computing degrees, one finds that $\Phi$ has tri-degree 
$(\lambda, \mu, \mu)$, with
\[
  \lambda = (d-2)(d^2-6)
  \quad \text{and}
  \quad
  \mu=d^3-2d^2+d-6.
\]
Since $\Phi$ is $\redDisc_d^2(f)$ with respect to the indeterminate
$\alpha$,
and the coefficient of $f(\alpha,\beta,\gamma)$ in
$\alpha^a\beta^b\gamma^c$
is a polynomial of degree $a$ in the indeterminates $p'$,
the fact that $\Phi$ is homogeneous in $p'$ and its
degree follow directly from \ref{pr:weight-reddisc.a}; to
wit, in our situation the degree in
\ref{pr:weight-reddisc.a} reads
\[
  d(d-1)^2-
  \bigl[ 7d  -12
  \bigr]
  = d^3-2d^2-6d+12
  = (d-2)(d^2-6).
\]
The homogeneity and degrees in $p$ and $p''$ however do not directly
follow from Proposition~\ref{pr:weight-reddisc}, as for instance the
coefficients in $A \beta^2 + 2B \beta\gamma + C \gamma ^2$ do not all
have the same weights in $p$ or $p''$. It is noticeable that 
$T^2A(B^2-AC)^2$ is homogeneous in $p$ and $p''$ because the weights
of $T^2$ and $A$ balance each other; this is a very elementary reason
why $T$ ``should'' appear with a square in Formula~\eqref{discr}.
The degree of $\redDisc_d^2(f)$ with the
weights as in \ref{pr:weight-reddisc.b} is
\[
2\bigl[
d(d-1)^2 - 6
\bigr]
= 2\bigl[
d^3-2d^2+d-6
\bigr],
\]
and one observes that its degrees in $p$ and $p''$ respectively are
one half of this, thus this degree ``distributes equally'' between $p$
and $p''$.


In conclusion, it follows as in Paragraph~\ref{p:divB^2-AC}
from Theorem~\ref{p:elim-lambdamumu} 
that there exists a homogeneous polynomial $K$ of degree 
$(d-2)(d^3-d^2+d-12)$
in the variable $p'$, with constant coefficients, such that for fixed
$p' \in S$ and $p'' \in \T_{p'}S$, $T$ divides $\Phi$
if and only if $K(p')=0$.

We have thus arrived at the following statement.

\begin{theorem}
\label{t:node-couple}
Let $S$ be a smooth, degree $d$, surface in $\P^3$.
There is a hypersurface $V(K)$ of degree $(d-2)(d^3-d^2+d-12)$, the
intersection of which with $S$ is the locus of tangency points of
planes bitangent to $S$.
\end{theorem}

It has to be recognized that the proof given above of the latter
statement rests on the not fully justified fact that $T$ divides $\Phi
= \redDisc(f)$ if and only if the tangent plane $\T_{p'}S$ is also
tangent to $S$ at some additional point.
The ``if'' part is established by
\cite[Theorem~\tref{t:dimca-tgcone}]{13.th-classic},
which is a result due to
Dimca \cite{dimca-16}, but what is really needed is the ``only if'' part.
Evidence in favour of that assertion is provided by the irreducibility
of the reduced discriminant $\Phi$
(which, as already mentioned, follows from the fact that the reduced discriminant is a toric discriminant; see also \cite{BD2}).
% : we have observed it for low values
% of $d$ with a computer algebra system, and prove it as a general
% statement in the follow-up article \cite{BD2}.

\begin{corollary}
\label{c:node-couple}
The ordinary double curve of the dual surface
$\dual S$ has degree 
$%\[
\frac 1 2 d(d-1)(d-2)(d^3-d^2+d-12).
$%\]
\end{corollary}

\begin{proof}
Let $p'' \in \P^3$ be a general point. The locus of those points $p' \in
S$ such that there exists a plane through $p''$ tangent to $S$ at $p'$ is
the apparent boundary $\polar {p''} S \cap S$.
Therefore, by Theorem~\ref{t:node-couple}, the locus of points 
$p'\in S$ such that $\T_{p'}S$ is bitangent and passes through $p''$ is
$\obspolar {p''} S \cap S \cap V(K)$.
Now for each bitangent plane there are two tangency points $p'$, so the
number of bitangent planes passing through $p''$ is
\[
\frac 1 2 \cdot \deg(S) \cdot 
\deg (\polar {p''} S) \cdot
\deg K.
\]
\end{proof}

\subsection{Generalization to hypersurfaces of arbitrary 
dimension}
\label{s:salmon-thecomput-arb}

In fact, Salmon's procedure works in arbitrary
dimension, using the generalization 
\eqref{eq:Salmonhypersurface} of formula \taylordisc.
The arguments are direct generalizations, so we are going to be sketchy.

\paragraph{}
Let $V=\V(F)$ be a smooth hypersurface of degree $d$ in $\P^n$, 
and consider $n$ points 
$p_1,\ldots,p_{n-1},p$ (or rather tuples $\hat p_1, \ldots, \hat
p_{n-1}, \hat p \in \k^{n+1}$).
The points $p_1,\ldots,p_{n-1}$ (if in linear general position,
\ie if $\hat p_1, \ldots, \hat p_{n-1}$ are linearly independent)
define a pencil of hyperplanes in $\P^n$,
and for all $p$ (not in $\vect{p_1,\ldots,p_{n-1}}$),
the tuples
$\hat p_1, \ldots, \hat p_{n-1}, \hat p$
define a system of homogeneous coordinates 
$(\alpha_1:\ldots:\alpha_{n-1}:\alpha)$ on the member $H_p$ of the
pencil determined by $p$, \ie
$\vect{p_1,\ldots,p_{n-1},p}$.
In this system of coordinates, the
hyperplane section $H_p \cap V$ is the zero locus of the polynomial
\begin{align*}
% \tilde f _{p_1,\ldots,p_{n-1},p} (\alpha_1,\ldots,\alpha_{n-1},\alpha)
  f (\alpha_1,\ldots,\alpha_{n-1},\alpha)
  &\overset{\text{def.}}=
    F (\alpha_1 \hat p_1 +\cdots +\alpha_{n-1} \hat p_{n-1}
    +\alpha \hat p)
  \\
  &= \sum_{k=0}^d \, \frac 1 {k!} \, \alpha_1^{d-k} \,
    \polar {(\alpha_2 \hat p_2 +\cdots +\alpha \hat p)^k}F (\hat p_1).
% \\ =
% T \alpha_1^{d-1} \alpha
% + \frac 1 2 \alpha_1^{d-2} \cdot
% \obspolar {(\alpha_2 \hat p_2 +\cdots +\alpha \hat p)^2} f(\hat p_1)
% \quad \mod (\alpha_2,\ldots,\alpha)^3,
\end{align*}
We shall assume that $p_1\in V$ and
$p_2,\ldots,p_{n-1} \in \T_{p_1}V$, equivalently
\[
  F(p_1) = \polar {p_2}F(p_1) = \cdots =  \polar {p_{n-1}}F(p_1) = 0.
\]
Then, 
\begin{align*}
  f (\alpha_1,\ldots,\alpha_{n-1},\alpha)
  = T \alpha_1^{d-1} \alpha
  + \frac 1 2 \alpha_1^{d-2} f_2(\alpha_2,\ldots,\alpha_n,\alpha)
  \quad \mod (\alpha_2,\ldots,\alpha)^3
\end{align*}
where $T=\obspolar {\hat p} f(\hat p_1)$
and
$f_2(\alpha_2,\ldots,\alpha_n,\alpha)
= \polar {(\alpha_2 \hat p_2 +\cdots +\alpha \hat p)^2} F(\hat p_1)$.
By Formula~\eqref{eq:Salmonhypersurface}, the generalization of
\taylordisc{}, one has
\begin{equation*}
  % \Disc (H_p \cap X)
  \Disc(f) = T^2\cdot \Disc(\bar f_2) \cdot
  \Disc(f_2)^2 \cdot \Phi \quad\mod T^3,
\end{equation*}
with $\bar f_2 (\alpha_2,\ldots,\alpha_n) = 
f_2(\alpha_2,\ldots,\alpha_n,0)$
and $\Phi = \redDisc_d^2(f)$.
Our task is to analyze the divisibilities of $\Disc(f_2)$ and
$\Phi$ by $T$
($\bar f_2$ has degree $0$ in $p$, hence $T$ divides
$\Disc(\bar f_2)$ if and only if $\Disc(\bar f_2)=0$).

\paragraph{}
% \label{p:adapt-linesInt}
\label{p:elim-aux-n}
Theorem~\ref{p:elim-lambdamumu} (Salmon's elimination trick)
generalizes as follows.
Given $n-1$ linear forms
$L_1,\ldots,L_{n-1} \in \P^n$, 
the line $\V(L_1,\ldots,L_{n-1})$ intersects the
$(n-2)$-dimensional linear space
$\vect {p_1,\ldots,p_{n-1}}$ if and only if
\begin{equation*}
D_{L_1,\ldots,L_{n-1}}(p_1,\ldots,p_{n-1})
\overset{\text{def.}}=
\det \bigl( L_i (p_j) \bigr) _{1\leq i,j \leq n-1}
\end{equation*}
vanishes.

Let
\[
\Tan V
:=\{ (p_1,\ldots,p_{n-1}) \in (\P^n)^{n-1}:
p_1\in V
\text{ and }
p_2,\ldots,p_{n-1} \in \T_{p_1}V
\},
\]
and consider a multihomogeneous polynomial 
$\Phi_{p_1,\ldots,p_{n-1}}(p)$ of multidegree $(\lambda,\mu,\ldots,\mu)$
in the sets of variables $p_1,\ldots,p_{n-1},p$, such that
for all $(p_1,\ldots,p_{n-1}) \in \Tan V$, the hypersurface
$\V(\Phi_{p_1,\ldots,p_{n-1}})$ consists of $\mu$ hyperplanes, counted
with multiplicities, all containing
the $(n-2)$-plane $\vect {p_1,\ldots,p_{n-1}}$.

Then, the locus of those $p_1 \in V$ such that there exist
$p_2,\ldots,p_{n-1} \in \T_{p_1}V$
such that
$\T_{p_1}X$ is a component of $\V(\Phi_{p_1,\ldots,p_{n-1}})$ is cut out
on $V$ by a hypersurface of degree $\lambda+\mu (d-2)$.

\bigskip\noindent
One may then argue as in \ref{p:lambdamumu-aux}
to analyze the divisibilities of $\Disc(f_2)$ and $\Phi$ by $T$.

\paragraph{}
\label{p:hess-arbdim}
For $\Disc(f_2)$, we find as before
that it is divisible by $T$ if and only if
$p_1$ lies on the Hessian hypersurface of $V$,
since $f_2 \pmod T$ defines the tangent cone at $p_1$ of 
the tangential hyperplane section $\T_{p_1}V \cap V$,
hence $\Disc(f_2)$ vanishes modulo $T$ if and only if
the latter tangent cone is singular, \ie if and only if $p_1$ is a
parabolic point of $V$.

And indeed $\Disc(f_2)$, being the determinant of the symmetric matrix
\[
\begin{pmatrix}
\polar {(p_2)^2} F(p_1) & \cdots & \polar {p_2p_{n-1}} F(p_1)
& \polar {p_2p} F(p_1) \\
\vdots & \ddots & \vdots & \vdots \\
\polar {p_{n-1}p_2} F(p_1) & \cdots & \polar {(p_{n-1})^2} F(p_1) &
\polar {p_{n-1}p} F(p_1) \\
\polar {pp_2} F(p_1) & \cdots & \polar {pp_{n-1}} F(p_1) &
\polar {p^2} F(p_1)
\end{pmatrix},
\]
has multidegree 
$\bigl((n-1)(d-2),2,\ldots,2\bigr)$ in
$p_1,\ldots,p_{n-1},p$, 
so the argument of \ref{p:elim-aux-n}
produces a homogeneous polynomial $H$ of degree 
\[
(n-1)(d-2)+2(d-2) = (n+1)(d-2)
\]
in the variable $p_1$.

\paragraph{}
The analysis of the divisibility of the reduced discriminant $\Phi$ by
$T$, on the other hand, 
gives rise to the couple-nodal polynomial $K$.

Let us first compute the multidegree of $\Phi$ in the variables
$p_1,\ldots,p_{n-1},p$. This goes as in
Paragraph~\ref{p:div-redDisc}.
First of all, $\Disc(f)$ is $n$-homogeneous of $n$-degree
$(\dual d,\ldots,\dual d)$ in $p_1,\ldots,p_{n-1},p$,
with $\dual d = d(d-1)^{n-1}$, hence so
is its homogeneous piece of lowest degree with respect to the Zariski
grading
\[
  T^2\, \Disc(\bar f_2)\, \Disc(f_2)^2\, \Phi.
\]
On the other hand, $T$ has  $n$-degree $(d-1,0,\ldots,0,1)$,
while
$\Disc(f_2)$ has $n$-degree $((n-1)(d-2),2,\ldots,2)$
as we saw in Paragraph~\ref{p:hess-arbdim} above.
The same computation gives the $n$-degree of $\Disc(\bar f_2)$, 
namely $((n-2)(d-2),2,\ldots,2,0)$.
Eventually, one finds that $\Phi$ has degrees
\[
d\bigl[(d-1)^{n-1}-1\bigr]-3(n-1)(d-2)
\quad \text{and} \quad
d(d-1)^{n-1}-6
\]
in $p_1$, and $p_2,\ldots,p_{n-1},p$, respectively
(note that the former degree is divisible by $d-2$).
As in Paragraph~\ref{p:div-redDisc}, the degree in $p_1$ of
$\redDisc_d^2(f)$ is given by
\ref{pr:weight-reddisc.a}, while the degree with respect
to the grading of \ref{pr:weight-reddisc.b} is equally
distributed between the degrees in $p_2,\ldots,p_{n-1},p$
respectively.

Eventually, by the result in Paragraph~\ref{p:elim-aux-n},
there exists a polynomial $K$ in $p_1$, homogeneous of degree
\[
d\bigl[(d-1)^{n}-1\bigr]-3(n+1)(d-2)
=(d-2) 
\Bigl(
d \cdot \frac {(d-1)^{n}-1} {d-2} -3(n+1)
\Bigr),
\]
such that $T$ divides $\Phi=\redDisc_d^2(f)$ if and only if $p_1 \in V$
lies on the hypersurface $\V(K)$. We call $K$ the couple-nodal
polynomial. 
One thus obtains the following result.

\begin{theorem}
\label{T:bitg-arbdim}
Let $V$ be a smooth degree $d$ hypersurface in $\P^n$, $n>1$.
The number of hyperplanes bitangent to $V$ passing through $n-2$ fixed
general points in $\P^n$ is
\begin{equation*}
\frac 1 2 d (d-1)^{n-2}
(d-2) 
\Bigl(
d \cdot \frac {(d-1)^{n}-1} {d-2} -3(n+1)
\Bigr).
\end{equation*}
\end{theorem}

For $n=3$ one recovers
Theorem~\ref{t:node-couple},
and for $n=2$ the number of bitangents to a smooth plane curve
of degree $d$,
viz.\ 
\begin{equation*}
\frac 1 2 (\dual d-1)(\dual d-2)
- 3d(d-2)
- \frac 1 2 (d-1)(d-2)
= \frac 1 2 d (d-2)(d-3)(d+3).
\end{equation*}


% \section{Two further enumerative computations}
% \label{S:further}

% In this final section we present two enumerative computations 
% for surfaces in $\P^3$, also
% taken from Salmon's book,
% which are close in spirit to the previous considerations. 


\section{Number of bitangent lines and generalizations}

In this section, we elaborate on the computation by Salmon of the
number of bitangent lines to a surface in $\P^3$ passing through a
general point. We give his proof in Section~\ref{s:bitg-lines}, and a
generalization to hypersurfaces in $\P^n$ in the next
Section~\ref{s:flex-bitg-lines}. These proofs only involve the reduced
discriminant of polynomials in two indeterminates, which is easily
expressed as a plain discriminant, see Example~\ref{ex:reddiscn=1}.
We give however another generalization in Section~\ref{s:bitg-colines},
for which it is necessary to consider reduced discriminants of
polynomials with an arbitrary number of indeterminates.
The two statements of Sections \ref{s:bitg-lines} and
\ref{s:flex-bitg-lines} are instances of a vast generalization by
Fehér and Juhász \cite{feher-juhasz}, which is described in
\cite[Theorem~\tref{t:feher-juhasz}]{14.th-vainsencher}.


\subsection{Number of bitangent lines}
\label{s:bitg-lines}

The Grassmannian of lines in $\P^3$ has dimension $4$. Passing through
a fixed point imposes $2$ conditions to a line in $\P^3$, and being
tangent to a surface (at an unprescribed point) imposes $1$ condition,
so one expects finitely many bitangent lines to a surface passing
through a general point in $\P^3$.
In this subsection we prove the following, along the lines of
\cite[\S 279]{salmon1}.

\begin{theorem}
\label{t:bitg-lines}
Let $S$ be a smooth surface of degree $d$ in $\P^3$, and $p \in \P^3$
a general point. The number of lines bitangent to $S$ and passing
through $p$ is
\begin{equation}
\label{nr:bitg-lines}
\frac 1 2 d (d-1)(d-2)(d-3).
\end{equation}
\end{theorem}

Salmon's strategy is similar in spirit to that exposed in
subsection~\ref{s:salmon-thecomput}. The fundamental fact is the
following. Consider as before
\[
\Tan S =\bigl\{ (p',p'') \in \P^3 \times \P^3: p'\in S \text{ and } p''
\in \T_{p'}S -\{p'\} \bigr\};
\]
equivalently, $(p',p'')$ is in $\Tan S$ if and only if $\vect
{p',p''}$ is a line, tangent to $S$ at $p'$.

\begin{proposition}
\label{pr:bitg-pol} There exists a polynomial $R$, bihomogeneous in
$p',p''$ with respective degrees $(d-2)(d-3)$ and $(d+2)(d-3)$, such
that the locus of points $(p',p'') \in \Tan S$ for which the line
$\vect {p',p''}$ is bitangent to $S$ is cut out on $\Tan S$ by
$V(R)$. 
\end{proposition}

\begin{proof}
Let $F$ be an equation of $S \subset \P^3$.
For $(p',p'') \in \Tan S$, we consider the homogeneous 
polynomial in $(\alpha,\beta)$
\begin{align}
\nonumber
  f(\alpha,\beta)
  & = F(\alpha p' + \beta p'')
  \\
\nonumber
  &= 
\alpha^d F(p') + \alpha^{d-1}\beta \polar {p''} F(p')
    + \frac 1 2 \alpha^{d-2}\beta^2  \polar {(p'')^2} F(p')
    + \cdots + \beta^d
F(p'')
\\ 
\label{eq:bitg-line}
&= \beta^2 \Bigl(
\frac 1 2 \alpha^{d-2} \polar {(p'')^2} F(p') + \cdots +
 \beta^{d-2} F(p'')
\Bigr)
\end{align}
(this is an abuse of notation: actually one should consider two
liftings $\hat p',\hat p'' \in \k^4$ of $p'$ and $p''$ respectively,
and $F(\alpha \hat p' + \beta \hat p'')$);
the last equality comes from the fact that $\vect
{p',p''}$ is tangent to $S$ at $p'$.
Let $\flat f (\alpha,\beta)$ be the homogeneous polynomial of degree
$d-2$ between parentheses at the right-hand-side of
\eqref{eq:bitg-line}.
The line $\vect {p',p''}$ is a bitangent to $S$ if and only if
$\flat f$ has a multiple root, so the polynomial $R$ we are looking
for is merely the discriminant of $\flat f$ which is none other, up
to sign, than the reduced discriminant of $f$, as noticed in
\ref{ex:reddiscn=1}.

Now, the polynomial $f$ is of the form
$$ f(\alpha,\beta)
= \beta^2\left(a_2\, \alpha^{d-2} + a_3\, \alpha^{d-3}\beta + \cdots
  a_d\, \beta^{d-2} \right)$$
where the coefficients $a_i$ are homogeneous in $p'$ and
$p''$ of degrees $d-i$ and $i$ respectively. Therefore, we deduce from
Example~\ref{ex:reddiscn=1} (see also Proposition~\ref{pr:weight-reddisc})
that $\redDisc(f)$ has degrees $(d-2)(d-3)$ and
$(d+2)(d-3)$ in $p'$ and $p''$ respectively, which concludes the proof.
\end{proof}


\begin{remark}
The degree of $\redDisc(f)$ in $p''$ may be computed alternatively as
follows. The plane curve $C_{p'} := \T_{p'} S \cap S$ has in general
a double point at $p'$, and what we want is the number of lines in
$\T_{p'} S$ passing through $p'$ and tangent to $C_{p'}$ at some other
point.  This is the number of ramification points of the projection of
$C_{p'}$ from $p'$; the latter is a $(d-2):1$ map $\bar C_{p'} \to
\P^1$, where $\bar C_{p'}$ denotes the normalization of $C_{p'}$
at $p'$, so
it follows from the Riemann--Hurwitz formula that the number of
ramification points equals
\begin{equation*}
2g(\bar C_{p'})-2+2(d-2)
= \bigl((d-1)(d-2)-2\bigr)-2+2(d-2)
= (d+2)(d-3)
\end{equation*}
as required.

We were not able to find, on the other hand, a geometric argument to
compute the degree in $p'$ in a comparable fashion. We wonder wether
there is an explanation to why this degree $(d-2)(d-3)$ is so nice, in
particular in its role in \eqref{nr:bitg-lines}.
It is conceivable
that it has something to do with the degree of the dual to a smooth
plane curve of degree $d-2$.
\end{remark}

\begin{proof}[Proof of Theorem~\ref{t:bitg-lines}]
Let $p \in \P^3$ be a general point. The locus of those points $p' \in
S$ such that $(p',p) \in \Tan S$ (equivalently, $p \in \T _{p'}
S$) is the apparent boundary $\polar p S \cap S$. Among these points
$p'$, the locus of those $p'$ for which the line $\vect {p,p'}$ is a
bitangent to $S$ is cut out by $V(R^p)$, where
$R^p = R(\_,p)$ with
$R$ the polynomial of
Proposition~\ref{pr:bitg-pol}; it is therefore a complete intersection
in $\P^3$ of type $(d,d-1,(d-2)(d-3))$. One concludes by observing
that there are two points $p'$ for every bitangent line to $S$
passing through $p$.
\end{proof}


\subsection{A generalization in arbitrary dimension}
\label{s:flex-bitg-lines}

The following is a fairly direct generalization of
Theorem~\ref{t:bitg-lines}; as we will see the proof is almost
identical to that of Salmon
for $n=2$ described in the previous subsection.

\begin{theorem}
\label{t:flex-bitg-lines}
Consider an integer $n > 3$.
Let $V$ be a smooth hypersurface of degree $d \geq n+1$ in $\P^n$, and
$p$ be a general point of $\P^n$.
The number of lines passing through $p$ and with two contact points
with $V$ of respective orders $2$ and $n-1$ is
\begin{equation}
\label{num:flex-bitg-lines}
  \prod\nolimits_{k=0}^n (d-k).
\end{equation}
\end{theorem}

To be precise, the lines under consideration in the above statement
are those lines $L$ in $\P^n$ such that the intersection scheme of $L$
with $V$ has the form
\[
  L\cap V = 2 p_1 +(n-1) p_2 + p_3 + \cdots + p_{d-n+1}.
\]
For $n=3$ this would be bitangent lines as in
Theorem~\ref{t:bitg-lines};
the reason why we assume $n>3$ above is because if $n=3$ the number
\eqref{num:flex-bitg-lines} actually counts ordered pairs of points
$(p_1,p_2)$ such that $\vect {p_1,p_2}$ is a bitangent line, so that
the number of bitangent lines is only one half of the number
\eqref{num:flex-bitg-lines}, as we have seen indeed in
Theorem~\ref{t:bitg-lines}.

The family of lines in $\P^n$ passing through $p$ has dimension $n-1$:
indeed, a line containing $p$ is uniquely determined by the datum of a
point in the projective quotient $\P^n/p$.\footnote
{\forcelabel{footnote}{projquot}
this abusive but suggestive notation has the following meaning:
if $\P^n = \P(\k^{n+1})$, and $\hat p \in \k^{n+1}$ represents $p\in
\P^n$, then $\P^n/p$ stands for the $(n-1)$-dimensional projective
space $\P\bigl( \k^{n+1}/ \vect {\hat p}\bigr)$.}
On the other hand an order $2$ contact (\ie an ordinary tangency) is
$1$ condition, and an order $n-1$ contact is $n-2$ conditions.
It is thus expected that the number of lines as in the theorem be
finite.


\begin{proof}[Proof of the theorem]
Consider
\[
  \Tan V =\{ (p',p'') \in \P^n \times \P^n:\quad
  p'\in V,\quad
  p'' \in \dD_{p'}V \cap \cdots \cap \dD_{{p'}^{n-2}}V,\quad
  \text{and}\quad p''\neq p'
  \}:
\]
the pair $(p',p'')$ is in $\Tan V$ if and only if $\vect
{p',p''}$ is a line, with contact of order $n-1$ with $V$ at $p'$,
see \cite[Theorem~\tref{t:polars-tglines}]{13.th-classic}.
For $(p',p'') \in \Tan S$, we consider the homogeneous 
polynomial in $(\alpha,\beta)$
\begin{align}
\nonumber
  f(\alpha,\beta)
  & = F(\alpha p' + \beta p'')
  \\
\nonumber
  &= 
\alpha^d F(p') + \alpha^{d-1}\beta \polar {p''} F(p')
    + \frac 1 2 \alpha^{d-2}\beta^2  \polar {{p''}^2} F(p')
    + \cdots + \beta^d F(p'')
\\ 
%\label{eq:flex-bitg-line}
&= \beta^{n-1} \Bigl(
\frac 1 {(n-1)!} \alpha^{d-n+1} \polar {{p''}^{n-1}} F(p') + \cdots +
 \beta^{d-n+1} F(p'')
\Bigr),
\end{align}
and denote by $\flat f (\alpha,\beta)$ the degree $d-n+1$ polynomial
between parentheses in the last expression.
The line $\vect {p',p''}$ has an additional tangent point with $V$ if
and only if the discriminant of $\flat f$ vanishes.
For all $i=n-1,\ldots,d$,
$\polar {{p''}^{i}} F(p')$ has degree $i$ in $p''$ and $d-i$ in $p'$.
Therefore, by Example~\ref{ex:reddiscn=1}, $\Disc(\flat f)$ has degree
$(d-n+1)(d-n)$
in $p'$.

Now, the locus of those points $p'\in V$ such that
$(p',p) \in \Tan V$,
\ie such that the line $\vect {p,p'}$ has contact of order $n-1$ with
$V$ at $p'$, is the intersection
$V \cap \dD^p V \cap \cdots \cap \dD^{p^{n-2}}$
(see \cite[Theorem~\tref{t:polars-tglines}]{13.th-classic}),
% or recall
% \cite[Display~\tref{{kth-polar-vs-polar-kic}}]{13.th-classic}),
which is the complete intersection of $n-1$ hypersurfaces of degrees
$d, d-1,\ldots,d-n+2$ respectively.
By the first part of the proof, those $p'$ such that the line
$\vect {p,p'}$ has an additional contact of order $2$ are cut out in
this complete intersection by an $n$-th equation, of degree
$(d-n+1)(d-n)$. One thus gets a $0$-dimensional complete intersection
of degree
\[
  d\, (d-1)\cdots (d-n+2) \bigl[
  (d-n+1)(d-n)
  \bigr],
\]
which is isomorphic to the family of lines we are interested in.
\end{proof}


\subsection{A dual generalization in arbitrary dimension}
\label{s:bitg-colines}

The family of codimension $2$ linear subspaces $\Lambda \subset \P^n$
passing through $n-2$ points $p_1,\ldots,p_{n-2}$ in linear general
position is isomorphic to $\P^2$:
indeed, such a linear subspace $\Lambda$ is uniquely determined by the
datum of a point 
in the $2$-dimensional projective quotient
\[
  \P^n/\vect{p_1,\ldots,p_{n-2}}
\]
(\ie
$\P\bigl( \k^{n+1} / \vect {\hat p_1,\ldots,\hat p_{n-2}}$,
see footnote~\ref{projquot}).
Besides, the Grassmannian of codimension $2$ linear subspaces in
$\P^n$ has dimension $2(n-1)$, and in this codimension passing through a
given point is given by two independent linear conditions.


In $\P^n/\vect{p_1,\ldots,p_{n-2}} \cong \P^2$,
those $\Lambda$ that are tangent to $V$ at one point
are parametrized by a curve $C$, and those that are bitangent to $V$
(\ie tangent at two points) are finitely many.
The degree of $C$ is readily computed; the theorem below gives the
number of bitangent codimension $2$ linear subspaces.

In Paragraph~\ref{p:tg-colines} below,
we explain how the degree of $C$ may
be found using homogeneity properties of the discriminant; we shall
see that the number of bitangent codimension $2$ subspaces involves
analogously a homogeneity property of the reduced discriminant.

\begin{theorem}
\label{t:bitg-colines}
Consider an integer $n \geq 3$.
Let $V$ be a general hypersurface of degree $d \geq 4$ in $\P^n$, and
$p_1,\ldots,p_{n-2}$ be points in linear general position in $\P^n$.
Then the number of codimension $2$ linear subspaces
$\Lambda \subset \P^n$
passing through $p_1,\ldots,p_{n-2}$ and bitangent to $V$ is
\begin{equation*}
%\label{num:bitg-colines}
  \frac 1 2
  \,d(d-1)^{n-2} (d-2)
  \,\frac
  {d(d-1)^{n-2}-(3n-5)d+6(n-2)}
  {d-2}.
\end{equation*}
\end{theorem}


\noindent
The peculiar way in which the formula is written is meant to emphasize
that $2$ is a root of the polynomial
$d(d-1)^{n-2}-(3n-5)d+6(n-2)$.

The transversality condition that must be satisfied by $V$ for the
formula to be valid is the following: $V$ must be smooth and have
finitely many bitangent codimension $2$ subspaces through general
points $p_1,\ldots,p_{n-2}$, each being tangent at only finitely many
points. If it happens that some bitangent
subspace has more than two ordinary tangency points, then it has to be
counted with the appropriate multiplicity.

We will not insist on verifying that the open subset of the linear
space of all degree $d$ hypersurfaces defined by this transversality
condition is indeed non-empty, but we will indicate where it is needed
in the proof.


\paragraph{}
\label{p:tg-colines}
The degree of the curve $C \subset \P^2 \cong
\P^n/\vect{p_1,\ldots,p_{n-2}}$ of simply tangent codimension $2$
subspaces is the number of its intersection points with 
a given line in $\P^2$;
it is also the number of $(n-2)$-planes $\Lambda \subset \P^n$ tangent to
$V$, passing through $p_1,\ldots,p_{n-2}$, and contained in a fixed
hyperplane $H$ which itself passes through $p_1,\ldots,p_{n-2}$.

The degree of $C$ may be computed using the homogeneity properties of
the (plain) discriminant.
Let $F \in \k[X_0,\ldots,X_n]$ be an equation of $V$. We consider the
polynomial $f \in \k[A,A_1,\ldots,A_{n-2}]$, depending on the
(implicit) parameters $p,p_1,\ldots,p_{n-2} \in \P^n$, defined by 
\[
  f(A,A_1,\ldots,A_{n-2})
  = F(A.p+A_1.p_1+\cdots + A_{n-2}.p_{n-2})
\]
(with the usual abuse of notation that we do not distinguish between
$p,p_1,\ldots,p_{n-2} \in \P^n$ and their representatives
$\hat p,\hat p_1,\ldots, \hat p_{n-2} \in \k^{n+1}$).
Then, 
\begin{multline*}
  f(A,A_1,\ldots,A_{n-2})
  = \\
  A^d F(p) + A^{d-1} \dD^{A_1.p_1+\cdots + A_{n-2}.p_{n-2}}F(p)
  +\, \cdots \, + \frac 1 {d!}
  \dD^{(A_1.p_1+\cdots + A_{n-2}.p_{n-2})^d}F(p)
\end{multline*}
by the Taylor--Newton formula,
and from this expression we see that the coefficient of $f$ in the
monomial $A^\alpha A_1^{\alpha_1}\cdots A_{n-2}^{\alpha_{n-2}}$ is
homogeneous of degree $\alpha$ in the parameter $p$.
Therefore, the discriminant $\Disc(f)$ is homogenous of degree
$d(d-1)^{n-2}$ in the parameter $p$,
by Proposition~\ref{par:weightdisc.a}.

The hypersurface in $\P^n$ defined by this homogeneous polynomial is
the cone of vertex $\vect{p_1,\ldots,p_{n-2}}$ swept out by those
$(n-2)$-planes $\vect{p,p_1,\ldots,p_{n-2}}$ that are tangent to $V$.
It projects from $\vect{p_1,\ldots,p_{n-2}}$ to the curve $C$ in
\(
\P^n/\vect{p_1,\ldots,p_{n-2}}
\cong \P^2
\),
hence $C$ has degree $d(d-1)^{n-2}$.

As we will see in the proof of Theorem~\ref{t:bitg-colines}, the
tangency points with $V$ of the $(n-2)$-planes parametrized by $C$
form
the complete intersection curve
$V\cap \polar {p_1} V \cap \cdots \cap \polar {p_{n-2}} V$,
which has degree $d(d-1)^{n-2}$ and projects birationally to $C$ from
$\vect{p_1,\ldots,p_{n-2}}$; this gives another way of computing the
degree of $C$.


\paragraph{Proof of Theorem~\ref{t:bitg-colines}}
% \begin{proof}
We continue with the setup introduced in \ref{p:tg-colines}
above, but now we assume that $p$ sits on $V$ and is such that the
$(n-2)$-plane $\vect{p,p_1,\ldots,p_{n-2}}$ is tangent to $V$ at $p$
itself; equivalently, $p$ sits on the complete intersection curve
$V\cap \polar {p_1} V \cap \cdots \cap \polar {p_{n-2}} V$.\footnote
{this equivalence needs the smoothness of $V$; the fact that this is a
complete intersection is equivalent to the fact that tangent subspaces
through $p_1,\ldots,p_{n-2}$ form a curve.}
Under this assumption, the polynomial $f$ takes the form
{\setlength{\multlinegap}{10mm}
\begin{multline*}
  f(A,A_1,\ldots,A_{n-2})
  = \\
  \frac 1 2 A^{d-2} \dD^{(A_1.p_1+\cdots + A_{n-2}.p_{n-2})^2}F(p)
  +\, \cdots \, + \frac 1 {d!}
  \dD^{(A_1.p_1+\cdots + A_{n-2}.p_{n-2})^d}F(p),
\end{multline*}
}%
and its coefficient in the
monomial $A^\alpha A_1^{\alpha_1}\cdots A_{n-2}^{\alpha_{n-2}}$ is
still homogeneous of degree $\alpha$ in the parameter $p$, if
non-zero.

The $(n-2)$-plane $\vect{p,p_1,\ldots,p_{n-2}}$ is bitangent to $V$ if
and only if the reduced discriminant $\redDisc_d^2(f)$ vanishes.
Thus, the locus of points $p\in V$ such that
$\vect{p,p_1,\ldots,p_{n-2}}$ is tangent to $V$ in two points
including $p$ is the complete intersection of the curve 
$V\cap \polar {p_1} V \cap \cdots \cap \polar {p_{n-2}} V$
with the hypersurface defined by $\redDisc_d^2(f)$ as a polynomial in
$p$.\footnote
{again, the fact that this is indeed a complete intersection is
  equivalent to the fact that bitangent subspaces through
  $p_1,\ldots,p_{n-2}$ are finitely many, and each of those is tangent
  to $V$ at only finitely many points;
multiple points in this complete intersection will occur if some
bitangent subspace has more than two ordinary tangency points with $V$.}
The latter is homogeneous of degree
$d(d-1)^{n-2}-(3n-5)d+6(n-2)$ by
\ref{pr:weight-reddisc.a}.
Therefore, the locus of tangency points of bitangent $(n-2)$-planes
through $p_1,\ldots,p_{n-2}$ has degree
\[
  d(d-1)^{n-2} \bigl[
  d(d-1)^{n-2}-(3n-5)d+6(n-2)
  \bigr].
\]
The result follows, since each bitangent $(n-2)$-plane is tangent in
two points.
\qed
% \end{proof}



\section{The flecnodal polynomial}
\label{S:flecnodal}

This is carried out by Salmon in \cite[\S 588]{salmon2_16},
with \cite[\S 473]{salmon2_16} as a
fundamental tool. This has already been revisited in modern standards
in \cite{BASW-16}, and actually extended there to
hypersurfaces in a projective space of arbitrary dimension, so we are
going to be brief.

\paragraph{The problem}
Let $S$ be a smooth surface in $\P^3$ of degree $d>1$.
For a general point $p \in S$, there are two lines having intersection
multiplicity at $p$ with $S$ strictly greater than $2$: these are the
tangent lines to the two smooth branches at $p$ of the curve
$\T_pS \cap S$, which has an ordinary double point at $p$;
thus these two lines intersect $S$ with multiplicity $3$ at $p$.

We shall see that those points $p \in S$ such that there is a line
intersecting $S$ with multiplicity strictly greater than $3$ at $p$ is
a curve $Fl(S)$, cut out on $S$ by a polynomial of degree $11d-24$. We
call this curve (respectively polynomial) the \emph{flecnodal} curve
(respectively polynomial) of $S$. 

At a general point $p$ of the flecnodal curve, the section of $S$ by its
tangent hyperplane $\T_pS$ is a curve with a non-degenerate double
point at $p$ (\ie a double point with tangent cone of maximal rank),
such that one of its two local branches has an inflection point at $p$.
In general, the tangent line to the latter branch meets $S$ with
multiplicity $4$ at $p$. 
Those points $p \in S$ such that the curve $\T_pS \cap S$ has a
tacnode (\ie a double point with local equation $y^2=x^4$) also belong
to the flecnodal curve: they are its intersection points with the
Hessian of $S$, and they are cuspidal points of the cuspidal double
curve of $\dual S$ (the latter curve parametrizes those hyperplanes
that cut out a cuspidal curve on $S$).


\bigskip
The following statement is in the spirit of reduced elimination
theory, with the polynomial $R$
(in the notation of the proposition)
playing the role of the
reduced resultant.
Here we are not prescribing individual multiplicities at the point $q$
for the polynomials $F,G,H$ as in the reduced resultant situation,
but rather a multiplicity for the ideal
they generate; then $R$ vanishes when the subscheme defined by this
ideal is larger than what is imposed by the hypothesis, as does
$\redRes$ in the reduced resultant situation.

\begin{proposition}[{\cite[\S 473]{salmon2_16}}]
\label{pr:Salmon-elim}
Let $F_q(p),G_q(p),H_q(p)$ be three bi-homogeneous polynomials in 
$p,q \in \P^3$, of bi-degrees
$(\lambda,\mu)$, $(\lambda',\mu')$, $(\lambda'',\mu'')$
respectively. We assume that for the general point $q \in \P^3$,
\begin{equation*}
\mult_q \bigl( \V(F_q,G_q,H_q) \bigr) = \lambda \lambda' \lambda''.
\end{equation*}
The locus of those $q \in \P^3$ such that $\V(F_q,G_q,H_q)$ contains a
point in addition to $q$ counted with multiplicity $\lambda \lambda'
\lambda''$ is the zero locus of a homogeneous polynomial
$R$ of degree
\begin{equation*}
%\label{eq:deg-cont-line}
\lambda'\lambda'' \mu + 
\lambda\lambda'' \mu' + 
\lambda\lambda' \mu''
-\lambda \lambda' \lambda''.
\end{equation*}
\end{proposition}

Of course, the condition that the scheme $\V(F_q,G_q,H_q)$ contains a
point in addition to $q$ is equivalent to its having positive
dimension.
Salmon claims that it is equivalent to the fact that
$\V(F_q,G_q,H_q)$ contains a line; we have not been able to prove
it, but this is not needed for the application.

\begin{proof}
We want to characterize when the scheme $\V(F_q,G_q,H_q)$ has positive
dimension. The idea is that this is equivalent to its having non-empty
intersection with any hyperplane.
So let $L$ be a non-zero linear form in $p$, and consider the
resultant $\Res(L,F_q,G_q,H_q)$.
It follows from the Poisson formula (see, \eg
\cite[Prop.~2.2]{BASW-16} and the references therein)
and our assumption on $F,G,H$ that there exists a
polynomial $R$ such that
\begin{equation}
\label{eq:Salmon-elim}
\Res(L,F_q,G_q,H_q) = L(q) ^{\lambda \lambda'\lambda''}
\cdot R(L,F_q,G_q,H_q).
\end{equation}
Computing degrees, one sees that $R$ is homogeneous of degree $0$ in
the coefficients of $L$, \ie 
it does not depend on $L$.
It follows that $V(F_q,G_q,H_q)$ has positive dimension if and only if 
$R(F_q,G_q,H_q)=0$.
Eventually, one computes the degrees of $R(F_q,G_q,H_q)$
using the identity \eqref{eq:Salmon-elim}.
\end{proof}

\begin{theorem}
\label{t:flecnodal}
Let $S$ be a smooth surface in $\P^3$ of degree $d$.
There exists a homogeneous polynomial $Fl$ of degree $11d-24$, such that
the locus of points $p \in S$ such that there is a line intersecting
$S$ with multiplicity at least $4$ in $p$ is cut out on $S$ by $\V(Fl)$.
\end{theorem}

\begin{proof}
Let $p \in S$. It follows from
\cite[Thm.~\tref{t:polars-tglines}]{13.th-classic}
that
there is a line intersecting $S$ with multiplicity at least $4$ in $p$
if and only if the three polar hypersurfaces
$\Polar_pS,\Polar_{p^2}S,\Polar_{p^3}S$
(respectively, the tangent plane, the polar quadric, and the polar
cubic of $S$ at $p$)
have a common point besides $p$,
and that this in turn is equivalent to their having a whole line in
common.

On the other hand,
$\Polar_pS,\Polar_{p^2}S,\Polar_{p^3}S$,
which have degrees $1,2,3$ respectively, intersect with multiplicity
$6$ at $p$ by
\cite[Cor.~\tref{c:inters-polars}]{13.th-classic}.
We are therefore in a position
to apply Proposition~\ref{pr:Salmon-elim}, with $(\lambda,\mu)$,
$(\lambda',\mu')$, $(\lambda'',\mu'')$ equal to $(1,d-1)$, $(2,d-2)$,
$(3,d-3)$ respectively. The result follows.
\end{proof}




%\clearpage
% \bibliographystyle{mysmf-alpha}
% \bibliography{enumP3}

\providecommand{\bysame}{\leavevmode\hbox to3em{\hrulefill}\thinspace}
\providecommand{\og}{``}
\providecommand{\fg}{''}
\providecommand{\smfandname}{and}
\providecommand{\smfedsname}{\'eds.}
\providecommand{\smfedname}{\'ed.}
\providecommand{\smfmastersthesisname}{M\'emoire}
\providecommand{\smfphdthesisname}{Th\`ese}



\begin{references}

\setcounter{footnote}{0}
\renewcommand{\thefootnote}{\alph{footnote}}
\begin{thebibliography}[Chapters in this Volume\footnote
  {see \url{https://www.math.univ-toulouse.fr/~tdedieu/\#enumTV}}]{III}

\let\bibitem\varbibitem

\bibitem[\tref{02.edoardo}]{02.edoardo}
Th.~Dedieu and E.~Sernesi,
\emph{Deformations of curves on surfaces}.

\bibitem[\tref{13.th-classic}]{13.th-classic}
Th.~Dedieu,
\emph{Some formulas for curves and surfaces in {$\mathbf{P}^3$}}.

\bibitem[\tref{14.th-vainsencher}]{14.th-vainsencher}
Th.~Dedieu,
\emph{Node polynomials for curves on surfaces}.

\end{thebibliography}

\begin{thebibliography}[External References]{99}

\bibitem{italEMS-16}
M.~Beltrametti, E.~Carletti, D.~Gallarati {\normalfont \smfandname} G.~{Monti
  Bragadin}, \emph{Lectures on curves, surfaces and projective varieties -- a
  classical view of algebraic geometry}, EMS Textbooks in Mathematics, European
  Mathematical Society, 2009, Original version issued in 2003.

\bibitem{BASW-16}
L.~Bus\'e, C.~D'Andrea, M.~Sombra {\normalfont \smfandname} M.~Weimann,
  \emph{The geometry of the flex locus of a hypersurface}, Pacific Journal of Mathematics \textbf{304} (2020), no.~2, 419--437.

\bibitem{BD2}
  L.~Busé {\normalfont \smfandname} Th.~Dedieu,
  \emph{Discriminants of hypersurfaces with prescribed ordinary
    singularities},
  in preparation.

\bibitem{BJ14}
L.~Bus\'e {\normalfont \smfandname} J.-P. Jouanolou, \emph{On the
  discriminant scheme of homogeneous polynomials}, Math. Comput. Sci.
  \textbf{8} (2014), no.~2, 175--234.

\bibitem{CT78}
P.~Cartier {\normalfont \smfandname} J.~Tate, \emph{Simple proof of the main
  theorem of elimination theory in algebraic geometry}, Enseign. Math. (2)
  \textbf{24} (1978), no.~3-4, 311--317.

\bibitem{CLO98}
D.~A. Cox, J.~B. Little {\normalfont \smfandname} D.~O'Shea, \emph{Using
  algebraic geometry}, Graduate texts in mathematics, Springer, New York, 1998.

\bibitem{demazure}
M.~Demazure, \emph{R\'esultant, discriminant}, Enseign. Math. (2) \textbf{58}
  (2012), no.~3-4, 333--373.

\bibitem{dimca-16}
A.~Dimca, \emph{Topics on real and complex singularities}, Advanced Lectures in
  Mathematics, Friedr. Vieweg \& Sohn, Braunschweig, 1987, An introduction.

% \bibitem{dolgachev-16}
% I.~V. Dolgachev, \emph{Classical algebraic geometry}, Cambridge University
%   Press, Cambridge, 2012, A modern view.

\bibitem{feher-juhasz}
  L.~M. Fehér {\normalfont \smfandname} A.~P. Juhász,
  \emph{Pl\"ucker formulas
    using equivariant cohomology of coincident root strata},
  arXiv:2312.06430.

\bibitem{FuTo04}
M.~Furuya {\normalfont \smfandname} M.~Tomari, \emph{A characterization of
  semi-quasihomogeneous functions in terms of the {M}ilnor number}, Proc. Amer.
  Math. Soc. \textbf{132} (2004), no.~7, 1885--1890.

\bibitem{GKZ-16}
I.~M. Gelfand, M.~M. Kapranov {\normalfont \smfandname} A.~V. Zelevinsky,
  \emph{Discriminants, resultants and multidimensional determinants}, Modern
  Birkh\"auser Classics, Birkh\"auser Boston, Inc., Boston, MA, 2008, Reprint
  of the 1994 edition.

\bibitem{harris_16}
J.~Harris, \emph{Algebraic geometry}, Graduate Texts in Mathematics, vol.~133,
  Springer-Verlag, New York, 1995, A first course.

\bibitem{hartshorne_16}
R.~Hartshorne, \emph{Algebraic geometry}, Springer-Verlag, New York-Heidelberg,
  1977, Graduate Texts in Mathematics, No.~52.

\bibitem{J91}
J.-P. Jouanolou, \emph{Le formalisme du r\'esultant}, Adv. Math. \textbf{90}
  (1991), no.~2, 117--263.

\bibitem{OM88}
E.~K. Ould~Mohamdi, \emph{\'Elimination r\'eduite}, \smfphdthesisname,
  Universit\'e de Strasbourg, 1988.

\bibitem{salmon1}
G.~Salmon, \emph{{A Treatise on the Analytic Geometry of Three Dimensions,
  Vol.~I}}, Chelsea Publishing Company, New York, 1958, reprint of the seventh
  (latest) edition.

\bibitem{salmon2_16}
\bysame, \emph{{A Treatise on the Analytic Geometry of Three Dimensions,
  Vol.~II}}, Chelsea Publishing Company, New York, 1965, reprint of the fifth
  (latest) edition.

\bibitem{salmon-inv}
\bysame,
\emph{Lessons introductory to the modern higher algebra},
Hodges, Foster and Co., Dublin, 1876, third edition.

\bibitem{vdW}
B.~L. van~der Waerden, \emph{Modern {A}lgebra. {V}ol.~{II}}, Frederick Ungar
  Publishing Co., New York, 1950, Translated from the third German edition.

\bibitem{zariski_16}
O.~Zariski, \emph{Generalized weight properties of the resultant of {$n+1$}
  polynomials in {$n$} indeterminates}, Trans. Amer. Math. Soc. \textbf{41}
  (1937), no.~2, 249--265.

\end{thebibliography}

\end{references}


% \medskip
\vfill
\noindent
Laurent Busé.
Université Côte d'Azur, Inria,
2004 route des Lucioles, 06902 Sophia Antipolis, France.
\href{mailto:laurent.buse@inria.fr}{laurent.buse@inria.fr}


\medskip\noindent
% Thomas Dedieu.
% Institut de Mathématiques de Toulouse~; UMR5219.
% Université de Toulouse~; CNRS.
% UPS IMT, F-31062 Toulouse Cedex 9, France.
Dedieu Thomas, Univ Toulouse, INUC, UT2J, INSA Toulouse, TSE, CNRS,
IMT, Toulouse, France.
\href{mailto:thomas.dedieu@math.univ-toulouse.fr}{thomas.dedieu@math.univ-toulouse.fr}

% \renewcommand{\thefootnote}{}
% \footnotetext{
% ThD was membre of project FOSICAV, which 
% has received funding from the European Union's Horizon
% 2020 research and innovation programme under the Marie
% Sk{\Poll}odowska-Curie grant agreement No~652782.}

\stopcontents[16.redres]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 

